Regularized Learning for Domain Adaptation under Label Shifts

We propose Regularized Learning under Label shifts (RLLS), a principled and a practical domain-adaptation algorithm to correct for shifts in the label distribution between a source and a target domain. We first estimate importance weights using labeled source data and unlabeled target data, and then train a classifier on the weighted source samples. We derive a generalization bound for the classifier on the target domain which is independent of the (ambient) data dimensions, and instead only depends on the complexity of the function class. To the best of our knowledge, this is the first generalization bound for the label-shift problem where the labels in the target domain are not available. Based on this bound, we propose a regularized estimator for the small-sample regime which accounts for the uncertainty in the estimated weights. Experiments on the CIFAR-10 and MNIST datasets show that RLLS improves classification accuracy, especially in the low sample and large-shift regimes, compared to previous methods.

==> 1-Introduction.tex <==
\section{Introduction}

In supervised learning, we usually make predictions on an unlabeled \emph{target} set by training a predictive model on a labeled \emph{source} set. This is a sensible approach especially when the source and target sets are expected to have i.i.d. samples from the same distribution. However, this assumption does not hold in many
real-world applications. 
%We want to demonstrate the problem of \emph{distributional shift} in two scenarios related to medical applications, while it arises in many other domains as well.
For example, often times predictions for medical diagnostics are based on data from a particular population of patients and machines due to the limited variety of data that is available in the
training phase. 

Let us consider the following scenario.
A classifier is trained to predict whether a patient has contracted a severe disease in country A based on the physical measurements and diagnosis (labeled source data). The disease is potentially even more prevalent in country B, where no experts are available to make a reliable diagnosis. 
%Most importantly, the diagnosis is currently made by the doctors using an unknown combination of symptom descriptions, measurements and other soft signals they can pick out. 
The following questions could be relevant in this scenario:
\begin{itemize}[leftmargin=1.5em ]
    \item If we send a group of volunteers to country B with the preliminary equipment to 
    record measurements of patients, how can the data in country A and the new unlabeled data from country B be used to
    update the classifier to give good diagnostic predictions for patients in country B?
    \item If our classifier diagnose a set of disease given a set of symptom in country A, can it also do well in a new country B?
    \item  can we use this data and update the model to diagnose disease better?%they just locally update
    \item If our group members visit the patients in country B in online and daily manner rather than batch and the disease is deadly, can the
    classifier be updated after only few patients have been measured, so as to maximize the
    accuracy of the diagnosis for the following patients?
    %If the diseases are dangerous and are needed to be diagnose quickly, can this group locally update the model online, patient after patient?
    % Similarly, the disease might spread very fast in country A after an unexpected event. Can we detect and adapt to the new disease distribution quickly when measuring the measurements one patient at a time? 
    %\fycomment{this could be merged with above point?}\Kamyar{Mathematically they are talking about the same thing}
\end{itemize}
Similar problems arise in many other domains besides health care, but we will use this medical example throughout the paper for ease of presentation.
% \fycomment{are we also discussing what is "good" (f-1 /accuracy etc. at some point?)}

If we view the data points $(X_i, Y_i)$ in the source and target set
as i.i.d. samples from a joint distributions $\disP$ and $\disQ$
taking values in $\X\times \Y$,
%% from each consisting of an input $x \in \X$ and a label $y$ in a finite domain $\Y$, as i.i.d. samples drawn from joint distributions $\disP$ and $\disQ$,
we are dealing with the \emph{distributional shift} problem when
$\disP \neq \disQ$. There are various ways to model the difference
between $\disP$ and $\disQ$, depending on the use case at
hand.%~\citet{scholkopf2012causal} studies
Traditionally, the two following perspectives are considered: (i)
the causal setting where the input $x$ explains the label $y$,
and $(ii)$ the anti-causal setting, where the label $y$ causes the input
$x$.

For the causal setting, one usually assumes
%the \emph{covariate shift}
that the marginal distribution of the covariates $x$ shifts
between $\disP$ and $\disQ$, whereas the conditional probability mass
function of $y$ given $x$ stays constant, which we denote as $p(y|x) =
q(y|x)$ for all $y\in \Y$ and $x\in \X$.
% This assumption is sensible when there is reason to believe that there is a true optimal mapping from $x$ to $y$ which
% does not change if the distribution of $x$ changes.  As an example,
% if a given set of symptoms correctly predicts a disease for the
% ``right reasons'', the predictive function should be the same, no
% matter which country you are moving to. Various methods have been developed in the extensive literature targeting the \emph{covariate shift} setting
% %has been studied extensively in the literature, 
% see e.g. importance weighting (reference), KMM, xyz~\citep{shimodaira2000improving}.
% Although many of these methods
% have theoretical guarantees, their dependence in the input dimension has made it 
% difficult to apply them to large datasets. Furthermore, going back to our motivating example, we can see that the causal setting alone does not capture the nature of many other practical use cases - that is, the covariate shift assumption is not satisfied.
Although this is valid in some situations, in many data science applications an inherent ground truth $Y$ causes an observation $X$.
%% there is an inherent ground truth $y$ that 
%% we want to learn given observations $x$, which can be "explained" by $y$. 
For example, reported physical symptoms might be approximately similar across all patients that have contracted a particular disease. This simplified
relation can be modeled 
%by the structural equation model (SEM) $x = f(y, \nu)$ where $\nu$ is independent noise or 
e.g. by a directed graphical model $Y \to X$. It is now possible that the percentage of ill patients in the two countries A and B are very different, i.e. $\disP(Y = y) \neq \disQ(Y=y)$ ($p(y) \neq q(y)$ for short) for all $y \in \Y$.  
Similarly, within one country, the number of ill patients may suddenly change because of an irregular event such as a natural catastrophe. 

\begin{wrapfigure}{t}{.35\textwidth}
% \begin{minipage}{1.\textwidth}
\vspace*{-.5cm}
  \centering
  \footnotesize
  \begin{tabular}{c|c}
    \multicolumn{1}{c}{Covariate Shift }&\multicolumn{1}{c}{Label Shift} \\
    \toprule
 \makecell{$p(x)\neq q(x)$\\$ p(y|x) = q(y|x)$}  & \makecell{$p(y)\neq q(y)$\\$ p(x|y) = q(x|y)$}\\
    \bottomrule
  \end{tabular}
  \vspace*{-.4cm}
%   \label{table:settings}
% \end{minipage}
\end{wrapfigure}

In all of the above cases, there is a shift in the distribution of the label $y$, while given a fixed label, the conditional distribution of $x$ given $y$ is constant, i.e., $p(x|y) = q(x|y)$.
By the Bayes rule, \emph{label shift} causes the covariate shift condition
to be violated, i.e.  $p(y|x) \neq q(y|x)$. Despite
being an intuitively natural scenario in some cases, even this simplified model has not yet been
sufficiently studied in the literature.
% In contrast to covariate shift,
% reweighting the samples in the source set is not straight-forward
% since the marginal distribution of $Y$ in distribution $\disQ$
% cannot be directly estimated.
%which is a gap we aim to fill with this work. 
This paper aims to fill the gap in terms of both theoretical understanding
and practical methods for the label shift setting and thereby move a step closer towards more complicated and realistic
distributional shift models. In particular, our goal was to find an efficient method which is scalable to large-scale data
where conventional approaches such as ones based on kernel mean embeddings, may become computationally feasible.

\cite{lipton2018detecting} introduced an importance-weight estimator, which has access to the labeled source data set and a large batch of unlabeled target data,
%(which we call the \emph{batch} setting), 
and demonstrated promising performance on real data. Using a black-box classifier which can be biased, uncalibrated and inaccurate, they first estimate importance weights $q(y)/p(y)$ for the source samples and train a classifier on the weighted data.
In the following we refer to the procedure as \emph{black box shift learning} (\zack{}) which the authors proved to be good for large enough sample size.
There are two relevant questions which remain unanswered by their work: What are the generalization guarantees for the final predictor which uses the weighted samples? How do we deal with the uncertainty of the weight estimation when only few samples are available?
%in the \emph{streaming} setting, when target samples come in one-by-one but it is still important to update the classifier even in the beginning when $\nq$ is very small?

In this work, our first contribution is to propose an efficient weight estimator for which we can obtain good statistical guarantees without a requirement on the problem-dependent minimum sample complexity as necessary for \zack{}, which in their case can be arbitrarily large for small number of samples. 
%in the finite-sample setting 
%We deploy this estimator and propose a label-shift correcting estimator and provide generalization guarantees. 
We then derive a dimension-independent generalization bound for the final Regularized Learning under Label Shift (\ose) classifier trained on the reweighted samples.
Our method improves the weight estimation error and the excess risk of the classifier on reweighted samples by a factor of $k\log(k)$, where $k$ is the number of classes, i.e. the cardinality of $\Y$. 
It also follows from our analysis that explicitly
%Depending on the number of source and target samples,
controlling the influence of our regularized weight estimates could help in practice. In particular, it suggests that when the number of target samples is 
below a certain threshold, the classifier would obtain higher accuracy if the weight estimates are not trusted because of high uncertainty and the samples stay unweighted.
%a threshold on the number of target samples above which a higher classification accuracy can be reached by reweighting the samples and below which the weights are still too uncertain to be used. 
% \fycomment{since we don't have a strictly better bound for smaller n (a constant of $\min (1, \theta_max)$ is not particularly great ...) I thought I should phrase the contribution in a more practical way}\Kamyar{you mean better than Zack's? the sample complexity?}
%and train a corrected classifier on the source set with the regularized weights.
% for the \ose estimator and show that its excess risk is bounded by $\Rade_n+\wt{\mathcal{O}}\left(\sqrt{{\log(k)}/{\np}}+\sqrt{{1}/{\nq}}\right)$ where $\Rade_n$ is the complexity of function class used for the training. To the best of our knowledge, this the first generalization bound for label shift problems where no knowledge about the labels in the target domain is assumed. Furthermore, for the low sample regime, when $\nq$ or $\np$ are small, we deploy these bounds and develop a regularization method for the importance weight estimation and further improve our generalization bound. \fycomment{needs to be adjusted when we have a clear agenda for the $\lambda$} 

We empirically study the performance of \ose and show weight estimation as well as prediction accuracy for a variety of shifts on the CIFAR-10 and MNIST datasets, including shifting source data and shifting target data with various parameters, different sample sizes and regularization parameters. We achieve an order of magnitude smaller weight estimation error than baseline methods in large shift cases and enjoy 20\% higher accuracy and F-1 score in corresponding predictive tasks. We also see at least 10\% accuracy improvement using our regularized estimator when faced with small target sample sizes.
% \Kamyar{ Are we going to share the Jupiter notebook of our code. Angie, if you confirm, we can state here "we also made our implementation public." }

%  In this work, we propose a statistically efficient way of estimating the importance weight which removes the warm-up sample complexity induced by \zack{} estimator. Moreover, we improved the estimation error in the importance weight estimation from direct linear dependence on $k$ in \zack{} to $\log(k)$.
% %the show that the error of our estimator grows by $\log(k)$ while the proposed estimator in \zack{} suffers from a linear dependence on $k$. 
% Besides providing a tight bound on the estimator, we derive a generalization bound on the batch learning under label shift problems, where we have fixed test sample size. We further extend this analysis to streaming of data when we start with no samples from the target and receive samples, one or mini-batch after another. We develop a regulation method in order to design an algorithm that guarantees high performance in the variety of sample size. We empirically study the significance of our weight estimator in a variety of different shifts. Under each scenario of different level of shifts, we deploy the estimated importance weight, train classifiers on the source data and evaluate its generalization on target data. 


==> 1-Introduction2.tex <==
\section{Introduction}


In many practical scenarios where  machine learning is employed, there can be big distributional shifts between the  data on which the model is trained (termed as the source distribution) and the data on which it is served (termed as the target distribution). Typically machine-learning models are trained on standard large-scale datasets,  and then served ``in the wild'' where data distribution can deviate widely and even be non-stationary. This is for example relevant in managed services on cloud providers 
or medical tools deployed in different regions in the world.
%such as Amazon Web Services~\citep{AWS}, Microsoft Azure~\citep{Azure}, and Google Cloud Platform~\citep{GCP}.
\fycomment{I don't like focusing on these too much. As if ML is only about those cloud services. In particular why name these platforms like an advertisement ...}
% \anima{cite web links to these}

%\anima{not a good idea to start paragraph with however}
Traditional supervised learning theory, however, assumes that both  training and testing data are independently and identically distributed (i.i.d.) according to the same distribution, and provides a bound on the generalization error under this assumption~\citep{mohri2012foundations}. Thus, there is a big gap in understanding generalization in practically relevant settings. \fycomment{what about Ben David's stuff? Vapnik/Bartlett...}   

%For example, survey response rates may vary by individuals' characteristics, different bias occurs in careless data collection process, labels from different sources carry noise, and label distribution constantly changes over time. These distribution shift scenarios make learning based on i.i.d assumption inappropriate and impose huge challenges for building reliable predictors in the wild.

\begin{wrapfigure}{t}{.35\textwidth}
% \begin{minipage}{1.\textwidth}
\vspace*{-.5cm}
  \centering
  \footnotesize
  \begin{tabular}{c|c}
    \multicolumn{1}{c}{Covariate Shift }&\multicolumn{1}{c}{Label Shift} \\
    \toprule
 \makecell{$p(x)\neq q(x)$\\$ p(y|x) = q(y|x)$}  & \makecell{$p(y)\neq q(y)$\\$ p(x|y) = q(x|y)$}\\
    \bottomrule
  \end{tabular}
  \vspace*{-.4cm}
%   \label{table:settings}
% \end{minipage}
\end{wrapfigure}

% \anima{please move causal and anti-causal to the end. it confuses amateurs.  }

In order to be able to derive efficient learning methods and make guarantees in the presence of distribution shifts between a source data distribution $\disP$ and a target data distribution $\disQ$, assumptions about the shift are necessary.
%to derive efficient domain-adaptation learning methods.
%\fycomment{first time domain-adaptation appears}
%\anima{introduce x and y} 
If we denote input variables as $x$ and output variables as $y$, we consider the two following settings: % are considered: 
(i) Covariate shift, which assumes that the conditional output distribution is invariant: $p(y|x) = q(y|x)$ between source and target distributions, but the source distribution $p(x)$ changes. (ii) Label shift,  where the conditional input distribution is invariant:  $p(x|y)=q(x|y)$ and  $p(y)$ changes from source to target. 

% \anima{use tilde before cite. it will keep it together}
The covariate shift scenario is challenging to handle for high-dimensional inputs $x$ such as images, videos and text, since precise density functions or generative models $p(x), q(x)$ are hard to obtain or learn. For example, importance weighting methods such as~\citep{shimodaira2000improving} require to learn a density (ratio) estimator beforehand, which is a difficult task on its own when the data is high-dimensional. The resulting generalization bounds based on importance weighting methods require the second order moments of the density ratio $(q(x)/p(x))^2$ to be bounded, which means the bounds are extremely loose in most cases
% \anima{what is impossible?}
~\citep{cortes2010learning}. 
\fycomment{I already tried to rephrase this but still don't quite get what the sentence is supposed to say} On the contrary, the label-shift problem is more tractable since the outputs $y$ is typically of a much lower dimension than $x$. Labels are usually either categorical variables with a finite number of categories or have simple well defined structures \fycomment{vague}, whose relation between source and target domain may be learned in an easier fashion
% \anima{could polish and say better}
. 
While covariate shift has been extensively studied in classical learning literature, the first label-shift estimation and correction framework has only been proposed recently~\citep{lipton2018detecting}. 

In some practical applications, the label-shift scenario is
of a greater concern. 
\fycomment{arguably more relevant.  - I wouldn't say more relevant, also relevant} 
For example, 
%cloud-providers and other suppliers of the machine-learning models have the resources to 
in some scenarios where machine learning models are used, 
they have to their disposal a large and a diverse source distribution to train the models that captures, to a large extent, the natural variations in the input $x$. On the other hand, they have no control on the proportion of label categories during test time. Another important scenario is the clinical applications, where the disease distribution changes over locations and time. Then the questions we are interested in are whether we can use data from source location or time period to predict disease in target location or time period in a efficient way. How many source and target data samples we need to obtain good performance on target data? Moreover, label shift can also be derived from the unconfounded anti-causal data generating model~\citep{scholkopf2012causal}: the label $y$ causes the input
$x$ and the causal mechanism that generates $x$
from $y$ is independent of the distribution of the $y$. But these causality assumptions are only special cases under which label shift holds. \fycomment{it's more like one way to derive it, or one perspective under which it makes sense. move somewhere later}
% Although covariate shift is much more investigated in literature, label shift naturally happens in many data science applications.
% %% there is an inherent ground truth $y$ that 
% %% we want to learn given observations $x$, which can be "explained" by $y$. 
% For example, reported physical symptoms might be approximately similar across all patients that have contracted a particular disease. This simplified
% relation can be modeled 
% %by the structural equation model (SEM) $x = f(y, \nu)$ where $\nu$ is independent noise or 
% e.g. by a directed graphical model $Y \to X$. It is now possible that the percentage of ill patients in the two countries A and B are very different, i.e. $p(y) \neq q(y)$ for all $y \in \Y$.  
% Similarly, within one country, the number of ill patients may suddenly change because of an irregular event such as a natural catastrophe.  

% Let us consider the following important scenario.
% A classifier is trained to predict whether a patient has contracted a severe disease in country A based on the physical measurements and diagnosis (labeled source data). The disease is potentially even more prevalent in country B, where no experts are available to make a reliable diagnosis. 
% %Most importantly, the diagnosis is currently made by the doctors using an unknown combination of symptom descriptions, measurements and other soft signals they can pick out. 
% The following questions are what we want to answer in this scenario:
% \begin{itemize}[leftmargin=1.5em ]
%     \item If we send a group of volunteers to country B with the preliminary equipment to 
%     record measurements of patients, how can the data in country A and the new unlabeled data from country B be used to
%     update the classifier to give good diagnostic predictions for patients in country B?
%     %\item If our classifier diagnose a set of disease given a set of symptom in country A, can it also do well in a new country B?
%     %\item  can we use this data and update the model to diagnose disease better?%they just locally update
%     \item If our group members visit the patients in country B in online and daily manner rather than batch and the disease is deadly, can the
%     classifier be updated after only few patients have been measured, so as to maximize the
%     accuracy of the diagnosis for the following patients?
%     %If the diseases are dangerous and are needed to be diagnose quickly, can this group locally update the model online, patient after patient?
%     % Similarly, the disease might spread very fast in country A after an unexpected event. Can we detect and adapt to the new disease distribution quickly when measuring the measurements one patient at a time? 
%     %\fycomment{this could be merged with above point?}\Kamyar{Mathematically they are talking about the same thing}
% \end{itemize}
% Similar problems arise in many other domains besides health care. For example, species distribution varies across different countries, which we need to take into account when learning to recognize them using images. Moreover, in topic classification using documents, topics distribution of news articles online constantly changes over time as well.


% \anima{i commented the healthcare application. the cloud framework is so much easier and less abstract. and everyone cares about it. u can add just 1-2 sentences in last para saying that there are other instances such as doing clinical studies in one country and selling the drug in another. Please re-write the questions directly in terms of x and y. no need for convoluted set of questions. }

% \anima{rewrite here.. that there is also a causality interpretation of these problems. cite scholkolf }
% $(i)$ 
% the causal setting where the input $x$ explains the label $y$,
% and $(ii)$ 


% For the causal setting, we usually assume
% %the \emph{covariate shift}
% that the marginal distribution of the covariates $x$ shifts
% between $\disP$ and $\disQ$, i.e. $p(x) \neq q(x)$, whereas the conditional label probability mass
% function of $y$ given $x$ stays constant, which we denote as $p(y|x) =
% q(y|x)$ for all $y\in \Y$ and $x\in \X$. While in the anti-causal setting, we usually assume the label $y$ shifts between $\disP$ and $\disQ$, i.e. $p(y) \neq q(y)$, whereas
% the conditional input distribution stays the same: $p(x|y) =
% q(x|y)$. Therefore, the former is called covariate shift and the the latter is called label shift.




%If we view the data points $(X_i, Y_i)$ in the source and target set
%as i.i.d. samples from a joint distributions $\disP$ and $\disQ$
%taking values in $\X\times \Y$,
%% from each consisting of an input $x \in \X$ and a label $y$ in a finite domain $\Y$, as i.i.d. samples drawn from joint distributions $\disP$ and $\disQ$,
%we are dealing with the \emph{distributional shift} problem when
%$\disP \neq \disQ$. There are various ways to model the difference
%between $\disP$ and $\disQ$, depending on the use case at
%hand.%~\citet{scholkopf2012causal} studies



%we usually make predictions on an unlabeled \emph{target} set by training a predictive model on a labeled \emph{source} set. This is a sensible approach especially when the source and target sets are expected to have i.i.d. samples from the same distribution. However, this assumption does not hold in many
%real-world applications. 
%We want to demonstrate the problem of \emph{distributional shift} in two scenarios related to medical applications, while it arises in many other domains as well.
%For example, often times predictions for medical diagnostics are based on data from a particular population of patients and machines due to the limited variety of data that is available in the
%training phase. 




% This assumption is sensible when there is reason to believe that there is a true optimal mapping from $x$ to $y$ which
% does not change if the distribution of $x$ changes.  As an example,
% if a given set of symptoms correctly predicts a disease for the
% ``right reasons'', the predictive function should be the same, no
% matter which country you are moving to. Various methods have been developed in the extensive literature targeting the \emph{covariate shift} setting
% %has been studied extensively in the literature, 
% see e.g. importance weighting (reference), KMM, xyz~\citep{shimodaira2000improving}.
% Although many of these methods
% have theoretical guarantees, their dependence in the input dimension has made it 
% difficult to apply them to large datasets. Furthermore, going back to our motivating example, we can see that the causal setting alone does not capture the nature of many other practical use cases - that is, the covariate shift assumption is not satisfied.


%In all of the above cases, there is a shift in the distribution of the label $y$, while given a fixed label, the conditional distribution of $x$ given $y$ is constant, i.e., $p(x|y) = q(x|y)$.
%By the Bayes rule, \emph{label shift} causes the covariate shift condition
%to be violated, i.e.  $p(y|x) \neq q(y|x)$. Despite
%being an intuitively natural scenario in some cases, even this simplified model has not yet been
%sufficiently studied in the literature.
% In contrast to covariate shift,
% reweighting the samples in the source set is not straight-forward
% since the marginal distribution of $Y$ in distribution $\disQ$
% cannot be directly estimated.
%which is a gap we aim to fill with this work. 
%\anima{weird sentence. modify} 
There are only few existing methods for label shift with access to labeled source data set and a large batch of unlabeled target data. ~\cite{zhang2013domain} proposed a kernel mean matching method for label shift, which requires kernel function evaluation and is not computationally feasible for large-scale data.
\fycomment{cite EM method McLachlan et al They estimate importance weight in label shift scenarios} Using importance weight estimates, 
~\cite{lipton2018detecting} introduced an estimator for the label shift setting
%(which we call the \emph{batch} setting), 
and demonstrated promising performance on large-scale data. Using a black-box classifier which can be biased, uncalibrated and inaccurate, they first estimate importance weights $q(y)/p(y)$ \fycomment{as in McLachlan} for the source samples and train a classifier on the weighted data.
In the following we refer to the procedure as \emph{black box shift learning} (\zack{}) which the authors proved to be good for large enough sample size.
However, there are two relevant questions which remain unanswered by their work: What are the generalization guarantees for the final predictor which uses the weighted samples? How do we deal with the uncertainty of the weight estimation when only few samples are available?
%in the \emph{streaming} setting, when target samples come in one-by-one but it is still important to update the classifier even in the beginning when $\nq$ is very small?

This paper aims to fill the gap in terms of both theoretical understanding
and practical methods for the label shift setting and thereby move a step closer towards a more complete \makeblue{literature} discourse on distribution shift \makeblue{problems} \fycomment{revisit sentence}. In particular, our goal is to find an efficient method which is applicable to large-scale data and to develop a good understanding of its generalization ability.

Our contribution in this work is trifold. Firstly, we propose an efficient weight estimator for which we can obtain good statistical guarantees without a requirement on the problem-dependent minimum sample complexity as necessary for \zack{}. In the \zack{} case, however, it can be arbitrarily large for a small number of samples. 
%This is enabled by a regularization technique motivated from theory \fycomment{weird statement - we use theory motivated by theory...?}.
%in the finite-sample setting 
%We deploy this estimator and propose a label-shift correcting estimator and provide generalization guarantees. 
Secondly, we derive a dimension-independent generalization bound for the final Regularized Learning under Label Shift (\ose) classifier based on the our weight estimator. 
In particular, our method improves the weight estimation error and the excess risk of the classifier on reweighted samples by a factor of $k\log(k)$, where $k$ is the number of classes, i.e. the cardinality of $\Y$. 
Finally, we propose a way to explicitly
%Depending on the number of source and target samples,
control the influence of our regularized weight estimates
in the low sample regime for the target data.
%, which could help to improve the performance when faced with low target sample size. S
More specifically, when the number of target samples is 
below a certain threshold, we show that the classifier would obtain higher accuracy if the weight estimates are less trusted \fycomment{I didn't like the "not trusted fully but are applied only partially or not applied" - too long, nor wanted to use "weight" here, have to think a bit more}, due to the possible high errors in weights.
%a threshold on the number of target samples above which a higher classification accuracy can be reached by reweighting the samples and below which the weights are still too uncertain to be used. 
% \fycomment{since we don't have a strictly better bound for smaller n (a constant of $\min (1, \theta_max)$ is not particularly great ...) I thought I should phrase the contribution in a more practical way}\Kamyar{you mean better than Zack's? the sample complexity?}
%and train a corrected classifier on the source set with the regularized weights.
% for the \ose estimator and show that its excess risk is bounded by $\Rade_n+\wt{\mathcal{O}}\left(\sqrt{{\log(k)}/{\np}}+\sqrt{{1}/{\nq}}\right)$ where $\Rade_n$ is the complexity of function class used for the training. To the best of our knowledge, this the first generalization bound for label shift problems where no knowledge about the labels in the target domain is assumed. Furthermore, for the low sample regime, when $\nq$ or $\np$ are small, we deploy these bounds and develop a regularization method for the importance weight estimation and further improve our generalization bound. \fycomment{needs to be adjusted when we have a clear agenda for the $\lambda$} 

In order to demonstrate benefit of the proposed method, we empirically study the performance of \ose and show weight estimation as well as prediction accuracy comparison for a variety of shifts on the CIFAR-10 and MNIST datasets, including shifting source data and shifting target data with various parameters, different sample sizes and regularization parameters. In large target sample cases when we apply regularized weights fully, we achieve an order of magnitude smaller weight estimation error than baseline methods in large shift cases and enjoy 20\% higher accuracy and F-1 score in corresponding predictive tasks. In low target sample cases when we apply regularized weights partially, we also see at least 10\% accuracy improvement over fully weighted and unweighted methods.
% \Kamyar{ Are we going to share the Jupiter notebook of our code. Angie, if you confirm, we can state here "we also made our implementation public." }

%  In this work, we propose a statistically efficient way of estimating the importance weight which removes the warm-up sample complexity induced by \zack{} estimator. Moreover, we improved the estimation error in the importance weight estimation from direct linear dependence on $k$ in \zack{} to $\log(k)$.
% %the show that the error of our estimator grows by $\log(k)$ while the proposed estimator in \zack{} suffers from a linear dependence on $k$. 
% Besides providing a tight bound on the estimator, we derive a generalization bound on the batch learning under label shift problems, where we have fixed test sample size. We further extend this analysis to streaming of data when we start with no samples from the target and receive samples, one or mini-batch after another. We develop a regulation method in order to design an algorithm that guarantees high performance in the variety of sample size. We empirically study the significance of our weight estimator in a variety of different shifts. Under each scenario of different level of shifts, we deploy the estimated importance weight, train classifiers on the source data and evaluate its generalization on target data. 


==> 1-Introduction3.tex <==
\section{Introduction}


In many practical scenarios where  machine learning is employed, there can be big distributional shifts between the  data on which the model is trained (termed as the source distribution) and the data on which it is served (termed as the target distribution). Typically machine-learning models are trained on standard large-scale datasets,  and then served ``in the wild'' where data distribution can deviate widely and even be non-stationary. This is for example relevant in managed services on cloud providers used by different clients, or medical tools deployed in different regions in the world. \Kamyar{I am not sure this last sentence add much, not clear to me how domain adaptation applies to these domain}\fycomment{don't you explain it in par. 4}
%such as Amazon Web Services~\citep{AWS}, Microsoft Azure~\citep{Azure}, and Google Cloud Platform~\citep{GCP}.
% \anima{cite web links to these}

%\anima{not a good idea to start paragraph with however}
Traditional supervised learning theory, however, assumes that both training and testing data are independently and identically distributed (i.i.d.) according to the same distribution, and provides a bound on the generalization error under this assumption~\citep{vapnik1999overview}. Thus, there is a big gap in understanding generalization in practically relevant settings. 

%For example, survey response rates may vary by individuals' characteristics, different bias occurs in careless data collection process, labels from different sources carry noise, and label distribution constantly changes over time. These distribution shift scenarios make learning based on i.i.d assumption inappropriate and impose huge challenges for building reliable predictors in the wild.

\begin{wrapfigure}{t}{.35\textwidth}
% \begin{minipage}{1.\textwidth}
\vspace*{-.5cm}
  \centering
  \footnotesize
  \begin{tabular}{c|c}
    \multicolumn{1}{c}{Covariate Shift }&\multicolumn{1}{c}{Label Shift} \\
    \toprule
 \makecell{$p(x)\neq q(x)$\\$ p(y|x) = q(y|x)$}  & \makecell{$p(y)\neq q(y)$\\$ p(x|y) = q(x|y)$}\\
    \bottomrule
  \end{tabular}
  \vspace*{-.4cm}
%   \label{table:settings}
% \end{minipage}
\end{wrapfigure}

% \anima{please move causal and anti-causal to the end. it confuses amateurs.  }
There are various ways to approach distribution shifts between a source data distribution $\disP$ and a target data distribution $\disQ$. If we denote input variables as $x$ and output variables as $y$, we consider the two following settings:
(i) Covariate shift, which assumes that the conditional output distribution is invariant: $p(y|x) = q(y|x)$ between source and target distributions, but the source distribution $p(x)$ changes. (ii) Label shift,  where the conditional input distribution is invariant:  $p(x|y)=q(x|y)$ and  $p(y)$ changes from source to target. 



Label-shift is a prominent scenario in a variety of practical machine learning applications. Considering the cloud-providers and other suppliers of the machine-learning models, they have the resources of large and diverse data sets (source set) to train the models, while, during the deployment, they have no control over the proportion of label categories during test time, e.g., ImageNet has the same number of American alligator as it has for car-wheel \citep{imagenet_cvpr09} while we see many cars but hopefully no alligator in the cities. Another important scenario is the clinical applications, where the disease distribution changes over locations and time. Considering the task of diagnosing disease based on the reported symptoms, the questions we are interested in are whether we can use data from source location or source time period to predict disease in target location or target time period in an efficient way. How many source and target data samples we need to obtain good performance on target data? Last but not the least, label shift also can be derived from the unconfounded anti-causal data generating model~\citep{scholkopf2012causal}: the label $y$ causes the input
$x$ and the causal mechanism that generates $x$
from $y$ is independent of the distribution of the $y$. But these causality assumptions are only special cases under which label shift holds. 


Covariate shift as another domain adaptation scenario is considered when there is a shift in the covariate distribution and conditional label distribution given covariates is unchanged. The principled study of covariate shift requires handling and estimation covariates density function  $p(x), q(x)$ which is infeasible in high-dimension, e.g., the covariate $x$ is an image, video, or text. For example, importance weighting methods such as~\citep{shimodaira2000improving} require to learn a density (ratio) estimator beforehand, which is a difficult task on its own when the data is high-dimensional. The resulting generalization bounds based on importance weighting methods require the second order moments of the density ratio $(q(x)/p(x))^2$ to be bounded, which means the bounds are extremely loose in most cases
% \anima{what is impossible?}
~\citep{cortes2010learning}. 
On the contrary, the label-shift problem is more tractable since the outputs $y$ is typically a much lower dimension than $x$. Labels are usually either categorical variables with a finite number of categories or have simple well-defined structures. 
Despite being an intuitively natural scenario in many real-world application, even this simplified model has not yet been sufficiently studied in the literature \citep{mclachlan2004discriminant,saerens2002adjusting}.


% Although covariate shift is much more investigated in literature, label shift naturally happens in many data science applications.
% %% there is an inherent ground truth $y$ that 
% %% we want to learn given observations $x$, which can be "explained" by $y$. 
% For example, reported physical symptoms might be approximately similar across all patients that have contracted a particular disease. This simplified
% relation can be modeled 
% %by the structural equation model (SEM) $x = f(y, \nu)$ where $\nu$ is independent noise or 
% e.g. by a directed graphical model $Y \to X$. It is now possible that the percentage of ill patients in the two countries A and B are very different, i.e. $p(y) \neq q(y)$ for all $y \in \Y$.  
% Similarly, within one country, the number of ill patients may suddenly change because of an irregular event such as a natural catastrophe.  

% Let us consider the following important scenario.
% A classifier is trained to predict whether a patient has contracted a severe disease in country A based on the physical measurements and diagnosis (labeled source data). The disease is potentially even more prevalent in country B, where no experts are available to make a reliable diagnosis. 
% %Most importantly, the diagnosis is currently made by the doctors using an unknown combination of symptom descriptions, measurements and other soft signals they can pick out. 
% The following questions are what we want to answer in this scenario:
% \begin{itemize}[leftmargin=1.5em ]
%     \item If we send a group of volunteers to country B with the preliminary equipment to 
%     record measurements of patients, how can the data in country A and the new unlabeled data from country B be used to
%     update the classifier to give good diagnostic predictions for patients in country B?
%     %\item If our classifier diagnose a set of disease given a set of symptom in country A, can it also do well in a new country B?
%     %\item  can we use this data and update the model to diagnose disease better?%they just locally update
%     \item If our group members visit the patients in country B in online and daily manner rather than batch and the disease is deadly, can the
%     classifier be updated after only few patients have been measured, so as to maximize the
%     accuracy of the diagnosis for the following patients?
%     %If the diseases are dangerous and are needed to be diagnose quickly, can this group locally update the model online, patient after patient?
%     % Similarly, the disease might spread very fast in country A after an unexpected event. Can we detect and adapt to the new disease distribution quickly when measuring the measurements one patient at a time? 
%     %\fycomment{this could be merged with above point?}\Kamyar{Mathematically they are talking about the same thing}
% \end{itemize}
% Similar problems arise in many other domains besides health care. For example, species distribution varies across different countries, which we need to take into account when learning to recognize them using images. Moreover, in topic classification using documents, topics distribution of news articles online constantly changes over time as well.


% \anima{i commented the healthcare application. the cloud framework is so much easier and less abstract. and everyone cares about it. u can add just 1-2 sentences in last para saying that there are other instances such as doing clinical studies in one country and selling the drug in another. Please re-write the questions directly in terms of x and y. no need for convoluted set of questions. }

% \anima{rewrite here.. that there is also a causality interpretation of these problems. cite scholkolf }
% $(i)$ 
% the causal setting where the input $x$ explains the label $y$,
% and $(ii)$ 


% For the causal setting, we usually assume
% %the \emph{covariate shift}
% that the marginal distribution of the covariates $x$ shifts
% between $\disP$ and $\disQ$, i.e. $p(x) \neq q(x)$, whereas the conditional label probability mass
% function of $y$ given $x$ stays constant, which we denote as $p(y|x) =
% q(y|x)$ for all $y\in \Y$ and $x\in \X$. While in the anti-causal setting, we usually assume the label $y$ shifts between $\disP$ and $\disQ$, i.e. $p(y) \neq q(y)$, whereas
% the conditional input distribution stays the same: $p(x|y) =
% q(x|y)$. Therefore, the former is called covariate shift and the the latter is called label shift.




%If we view the data points $(X_i, Y_i)$ in the source and target set
%as i.i.d. samples from a joint distributions $\disP$ and $\disQ$
%taking values in $\X\times \Y$,
%% from each consisting of an input $x \in \X$ and a label $y$ in a finite domain $\Y$, as i.i.d. samples drawn from joint distributions $\disP$ and $\disQ$,
%we are dealing with the \emph{distributional shift} problem when
%$\disP \neq \disQ$. There are various ways to model the difference
%between $\disP$ and $\disQ$, depending on the use case at
%hand.%~\citet{scholkopf2012causal} studies



%we usually make predictions on an unlabeled \emph{target} set by training a predictive model on a labeled \emph{source} set. This is a sensible approach especially when the source and target sets are expected to have i.i.d. samples from the same distribution. However, this assumption does not hold in many
%real-world applications. 
%We want to demonstrate the problem of \emph{distributional shift} in two scenarios related to medical applications, while it arises in many other domains as well.
%For example, often times predictions for medical diagnostics are based on data from a particular population of patients and machines due to the limited variety of data that is available in the
%training phase. 




% This assumption is sensible when there is reason to believe that there is a true optimal mapping from $x$ to $y$ which
% does not change if the distribution of $x$ changes.  As an example,
% if a given set of symptoms correctly predicts a disease for the
% ``right reasons'', the predictive function should be the same, no
% matter which country you are moving to. Various methods have been developed in the extensive literature targeting the \emph{covariate shift} setting
% %has been studied extensively in the literature, 
% see e.g. importance weighting (reference), KMM, xyz~\citep{shimodaira2000improving}.
% Although many of these methods
% have theoretical guarantees, their dependence in the input dimension has made it 
% difficult to apply them to large datasets. Furthermore, going back to our motivating example, we can see that the causal setting alone does not capture the nature of many other practical use cases - that is, the covariate shift assumption is not satisfied.


%In all of the above cases, there is a shift in the distribution of the label $y$, while given a fixed label, the conditional distribution of $x$ given $y$ is constant, i.e., $p(x|y) = q(x|y)$.
%By the Bayes rule, \emph{label shift} causes the covariate shift condition
%to be violated, i.e.  $p(y|x) \neq q(y|x)$. Despite
%being an intuitively natural scenario in some cases, even this simplified model has not yet been
%sufficiently studied in the literature.
% In contrast to covariate shift,
% reweighting the samples in the source set is not straight-forward
% since the marginal distribution of $Y$ in distribution $\disQ$
% cannot be directly estimated.
%which is a gap we aim to fill with this work. 
%\anima{weird sentence. modify} 
There are only few existing methods for label shift with access to labeled source data set and a large batch of unlabeled target data. ~\cite{zhang2013domain} proposed a kernel mean matching method for label shift, which requires kernel function evaluation and is not computationally feasible for large-scale data. Using importance weight estimates, 
~\cite{lipton2018detecting} deploys an estimator for the label shift setting
%(which we call the \emph{batch} setting), 
and demonstrated promising performance on large-scale data similar to \citet{mclachlan2004discriminant}. Using a black-box classifier which can be biased, uncalibrated and inaccurate, they first estimate importance weights $q(y)/p(y)$ for the source samples and train a classifier on the weighted data.
In the following we refer to the procedure as \emph{black box shift learning} (\zack{}) which the authors proved to be good for large enough sample size.
However, there are three relevant questions which remain unanswered by their work: How to estimate the importance weights in low sample setting, What are the generalization guarantees for the final predictor which uses the weighted samples? How do we deal with the uncertainty of the weight estimation when only few samples are available?
%in the \emph{streaming} setting, when target samples come in one-by-one but it is still important to update the classifier even in the beginning when $\nq$ is very small?

This paper aims to fill the gap in terms of both theoretical understanding
and practical methods for the label shift setting and thereby move a step closer towards a more complete literature discourse on distribution shift \makeblue{problems} \fycomment{revisit sentence}. In particular, our goal is to find an efficient method which is applicable to large-scale data and to develop a good understanding of its generalization ability.

Our contribution in this work is trifold. Firstly, we propose an efficient weight estimator for which we can obtain good statistical guarantees without a requirement on the problem-dependent minimum sample complexity as necessary for \zack{}. In the \zack{} case, however, it can be arbitrarily large for a small number of samples. 
%This is enabled by a regularization technique motivated from theory \fycomment{weird statement - we use theory motivated by theory...?}.
%in the finite-sample setting 
%We deploy this estimator and propose a label-shift correcting estimator and provide generalization guarantees. 
Secondly, we derive a dimension-independent generalization bound for the final Regularized Learning under Label Shift (\ose) classifier based on our weight estimator. 
In particular, our method improves the weight estimation error and the excess risk of the classifier on reweighted samples by a factor of $k\log(k)$, where $k$ is the number of classes, i.e. the cardinality of $\Y$. 
Finally, we propose a way to explicitly
%Depending on the number of source and target samples,
control the influence of our regularized weight estimates
in the low sample regime for the target data.
%, which could help to improve the performance when faced with low target sample size. S
More specifically, when the number of target samples is 
below a certain threshold, we show that the classifier would obtain higher accuracy if the weight estimates are less trusted \fycomment{I didn't like the "not trusted fully but are applied only partially or not applied" - too long, nor wanted to use "weight" here, have to think a bit more}, due to the possible high errors in weights.
%a threshold on the number of target samples above which a higher classification accuracy can be reached by reweighting the samples and below which the weights are still too uncertain to be used. 
% \fycomment{since we don't have a strictly better bound for smaller n (a constant of $\min (1, \theta_max)$ is not particularly great ...) I thought I should phrase the contribution in a more practical way}\Kamyar{you mean better than Zack's? the sample complexity?}
%and train a corrected classifier on the source set with the regularized weights.
% for the \ose estimator and show that its excess risk is bounded by $\Rade_n+\wt{\mathcal{O}}\left(\sqrt{{\log(k)}/{\np}}+\sqrt{{1}/{\nq}}\right)$ where $\Rade_n$ is the complexity of function class used for the training. To the best of our knowledge, this the first generalization bound for label shift problems where no knowledge about the labels in the target domain is assumed. Furthermore, for the low sample regime, when $\nq$ or $\np$ are small, we deploy these bounds and develop a regularization method for the importance weight estimation and further improve our generalization bound. \fycomment{needs to be adjusted when we have a clear agenda for the $\lambda$} 

In order to demonstrate benefit of the proposed method, we empirically study the performance of \ose and show weight estimation as well as prediction accuracy comparison for a variety of shifts on the CIFAR-10 and MNIST datasets, including shifting source data and shifting target data with various parameters, different sample sizes and regularization parameters. In large target sample cases when we apply regularized weights fully, we achieve an order of magnitude smaller weight estimation error than baseline methods in large shift cases and enjoy 20\% higher accuracy and F-1 score in corresponding predictive tasks. In low target sample cases when we apply regularized weights partially, we also see at least 10\% accuracy improvement over fully weighted and unweighted methods.
% \Kamyar{ Are we going to share the Jupiter notebook of our code. Angie, if you confirm, we can state here "we also made our implementation public." }

%  In this work, we propose a statistically efficient way of estimating the importance weight which removes the warm-up sample complexity induced by \zack{} estimator. Moreover, we improved the estimation error in the importance weight estimation from direct linear dependence on $k$ in \zack{} to $\log(k)$.
% %the show that the error of our estimator grows by $\log(k)$ while the proposed estimator in \zack{} suffers from a linear dependence on $k$. 
% Besides providing a tight bound on the estimator, we derive a generalization bound on the batch learning under label shift problems, where we have fixed test sample size. We further extend this analysis to streaming of data when we start with no samples from the target and receive samples, one or mini-batch after another. We develop a regulation method in order to design an algorithm that guarantees high performance in the variety of sample size. We empirically study the significance of our weight estimator in a variety of different shifts. Under each scenario of different level of shifts, we deploy the estimated importance weight, train classifiers on the source data and evaluate its generalization on target data. 


==> 2-RelatedWork.tex <==
\section{Related Work}
% This assumption is sensible when there is reason to believe that there is a true optimal mapping from $x$ to $y$ which
% does not change if the distribution of $x$ changes.  As an example,
% if a given set of symptoms correctly predicts a disease for the
% ``right reasons'', the predictive function should be the same, no
% matter which country you are moving to. Various methods have been developed in the extensive literature targeting the \emph{covariate shift} setting
% %has been studied extensively in the literature, 
% see e.g. importance weighting (reference), KMM, xyz~\citep{shimodaira2000improving}.
% Although many of these methods
% have theoretical guarantees, their dependence in the input dimension has made it 
% difficult to apply them to large datasets. Furthermore, going back to our motivating example, we can see that the causal setting alone does not capture the nature of many other practical use cases - that is, the covariate shift assumption is not satisfied.
The task of being robust against distributional shifts has been widely studied in the literature. One line of work focuses on distributional robustness (see e.g.~\cite{esfahani2017data, namkoong2016stochastic}) without explicitly modeling the shift by making assumptions on the distribution. Our theoretical results adapt to any shift $\theta$.
% \fycomment{not sure this is needed and requires a lot of rewriting since it's not quite understandable to me... there are a lot of works in distributional robustness in all sorts of dist. measures. I would mention them but not describe in such detail.}
% Furthermore, learning classifiers such that robustness to small perturbations in the probability space is guaranteed is studied when the perturbation is within a small \textit{Wasserstein} ball~\citep{esfahani2017data}. This notion of robustness is also extended to  the setting where importance weights in the loss are slightly perturbed around uniform in \textit{f-divergence} measure. The robustness is guaranteed when the perturbation shrinks linearly as the number of samples in the source increases. Moreover, robustness to a small and bounded convex set of given statistics also investigates where the explicit $\disQ(X)/\disP(X)$ needs to be computed. 
However, these methods achieve robustness only against tiny changes in the distribution and are often impractical for large-scale high dimensional data. %, while some of their assumptions are violated even in simple settings.
% \fycomment{} Therefore they are not suitable for label shift where the problems can be high dimensional and the shift are simply beyond their requirement. 
% \Kamyar{Not sure this discussion is required}

Another line of work has addressed the causal setting where the conditional distribution of $Y$ given $X$ is assumed to be constant. This assumption is sensible when there is reason to believe that there is a true optimal mapping from $X$ to $Y$ which
does not change if the distribution of $X$ changes. For example, in disease diagnosing problem,
if a given set of symptoms correctly predicts a disease for the
``right reasons'', the predictive function should be the same, no
matter which domain/location we deploy it.
Among the various methods to correct for covariate shift, 
the majority uses the concept of importance weights $q(x)/p(x)$  \citep{zadrozny2004learning,cortes2010learning,cortes2014domain,shimodaira2000improving}, which are unknown but can be estimated for example via kernel embeddings \citep{huang2007correcting,gretton2009covariate,gretton2012kernel,zhang2013domain,zaremba2013b} or by learning a binary discriminative classifier between source and target \citep{lopez2016revisiting,liu2017trimmed}. A minimax approach that aims to be robust to the worst-case shared conditional label distribution between source and target is also investigated~\citep{liu2014robust,chen2016robust}. Finally,~\citet{sanderson2014class,ramaswamy2016mixture} formulate the label shift problem as a mixture of the class conditional covariate distributions with unknown mixture weights. Under the pairwise mutual irreducibility~\citep{scott2013classification} assumption on the class conditional covariate distributions, they deploy the Neyman-Pearson criterion~\citep{blanchard2010semi} to estimate the class distribution $q(y)$. Class ratio estimation is also investigated in the maximum mean discrepancy framework~\citep{iyer2014maximum}.
% \fycomment{I don't think we need the detail ->}
% In order to relax the model assumption, a heuristic discrimination method using kernel logistic regression is deployed while suffers from lack of theoretical justification for the choice of importance weight estimates.
%
%\citep{zadrozny2004learning,cortes2014domain,shimodaira2000improving}.
%
% Domain adaptation through applying $\disQ(X)/\disP(X)$ \citep{zadrozny2004learning,cortes2014domain,shimodaira2000improving} is a prevalent approach to correcting covariate shift for low-dimensional data due to its (asymptotic) unbiasness. 
% \fycomment{not sure what the approach is - how is it applied? and why low-dimensional - so don't know whether I put the first set of references into the right place?}\angie{These are just old works on apply importance weights q(x)/p(x) on samples on covariate shift}
%
% However, it is well-known to require assumptions that are usually hard to satisfy in practice for high-dimensional data, like $\disQ(X)>0 \implies \disP(X) >0$ and bounded weights (norms) \citep{cortes2010learning}.  Previous work on density (ratio) estimation focus on overcoming the difficulty of obtaining good estimator by deploying kernel embedding of distribution in order to directly estimate $\disQ(X)/\disP(X)$ \citep{zhang2013domain,gretton2012kernel,zaremba2013b}, by learning a binary discriminative classifier using source and target data \citep{lopez2016revisiting} and by trimming extreme values for robust estimation \citep{liu2017trimmed}. 
Common issues shared by these methods is that they either result in a massive computational burden for large scale problems or cannot be deployed for neural networks. 
%Moreover, inaccurate estimates make classifiers suffer from high variance.

% around the source distribution  is mainly studies under diffrent notion of closenes,  constraint  of \textit{f-divergence}

% on small shifts is studied  Another perspective other than estimating density (ratio) directly is taking the adversarial approach by regarding density weights \citep{namkoong2016stochastic}, conditional label distribution\citep{liu2014robust} or samples \citep{esfahani2017data} as coming from a adversarial player in a minimax game. These methods aim to give distributionally robust predictions and benefit from worst-case guarantees.

% \fycomment{i'm guessing - also not scalable?} \angie{not quite sure about scalability here, but they are from different perspectives and are either covariate shift or not specific in shift type}

% Although the aforementioned previous works provide fundamental theoretical understanding and characterization of the covariate shift assumption, many of them require to explicitly estimate a notion of probability over $\X$ which prevent them from becoming applicable in the high dimensional data regime. Furthermore, as mentioned in the introduction, the assumption is violated in many problems where there is a distributional shift in $x$ but also $y$. 

Despite the wide applicability of label shift, approaches with global guarantees in high dimensional data regimes remain under-explored. The correction of label shift mainly requires to estimate the importance weights $q(y)/p(y)$ over the labels which typically live in a very low-dimensional space. %Since labels from the target domain are missing, this study stays challenging. 
Bayesian and probabilistic approaches are studied when a prior over the marginal label distribution is assumed \citep{storkey2009training, chan2005word}.
However, these methods often require explicitly computing the posterior distribution of $y$ and suffer from the curse of dimensionality.
% Then the observed $x$ from the target domain is used to compute the posterior over $q(y)$ which requires to explicitly construct $\disQ(X|Y)$, i.e.  unfeasible in high dimensions. Moreover, a hill climbing method, such as Expectation Maximization with the same motivation is employed to estimate $\disQ(Y)$ while still suffers from explicit construction of $\disQ(X|Y)$ \citep{chan2005word}. 
Recently, for the label shift setting, \citet{lipton2018detecting} proposed Black Box Shift Estimation (\zack) which can be applied to large scale data. This approach is related to \cite{buck1966comparison,forman2008quantifying,saerens2002adjusting} in the low dimensional setting but lacks guarantees for the excess risk.

On the other hand, generalization theory, usually used to bound the excess loss, has historically been developed for the case when $\disP=\disQ$ (see e.g.  \cite{vapnik1999overview,bartlett2002rademacher,kakade2009complexity,wain19}). \citet{ben2010theory} provides theoretical analysis and generalization guarantees for distribution shifts when the H-divergence between joint distributions is considered,  whereas \citet{crammer2008learning} proves generalization bounds for learning from multiple sources. For the covariate shift setting, \citet{cortes2010learning} provides a generalization bound when $q(x)/p(x)$ is known which however does not apply in practice.
% . However, in practical settings in high dimensions, this ratio is neither known nor bounded \fycomment{feasible to contract?}. The author provided a further analysis and relaxed the boundedness assumption at the cost of weaker bound. 


 
%  \fycomment{This paragraph should be merged to the Contributions section above. Here I would just write 1-2 sentences about what our major improvements compared to their paper are.}
%  In this work, we propose a statistically efficient way of estimating the importance weight which removes the warm-up sample complexity induced by \zack{} estimator. Moreover, we improved the estimation error in the importance weight estimation from direct linear dependence on $k$ in \zack{} to $\log(k)$.
% %the show that the error of our estimator grows by $\log(k)$ while the proposed estimator in \zack{} suffers from a linear dependence on $k$. 
% Besides providing a tight bound on the estimator, we derive a generalization bound on the batch learning under label shift problems, where we have fixed test sample size. We further extend this analysis to streaming of data when we start with no samples from the target and receive samples, one or mini-batch after another. We develop a regulation method in order to design an algorithm that guarantees high performance in the variety of sample size. We empirically study the significance of our weight estimator in a variety of different shifts. Under each scenario of different level of shifts, we deploy the estimated importance weight, train classifiers on the source data and evaluate its generalization on target data. \Kamyar{ Are we going to share the Jupiter notebook of our code. Angie, if you confirm, we can state here "we also made our implementation public." }


==> 3-Preliminaries.tex <==
\section{Preliminaries}
We denote $\X$ as the space of input and $\Y$ as categorical space of labels $\Y=\left[k\right]=\lbrace 1,\ldots,k\rbrace$ as a set of classes/categories.  We express the joint distribution input-label $(x,y)\in \X\times\Y$ in source domain $\S$ as $\disP$ and in target domain $\T$ as $\disQ$. Let us denote the marginal probability mass functions of $Y$ for
$\disP, \disQ$ shorthand as $p, q: [k] \to [0,1]$ with $p(i) = \disP(Y
= i)$, and $q(i) = \disQ(Y= i)$ for all $i \in [k]$, representable by vectors in $\Real_+^k$ which sum to one.


Correspondingly, we denote $p$ and $q$ as the marginal probability mass functions over labels in the source and the target domain, while the data set of samples from source is denoted as $D_p$ and for target as $D_q$. It worth noting that $D_q$ does not contain labels of target set. The cardinally of source data set is depicted as $n$ and for target as $m$ unless specified otherwise. Moreover, we use $\D_p(\X)$ as the marginal distribution of inputs in source as well as $\D_q(\X)$ for target. 

\paragraph{Problem set-up}
Let $h_0$ denote as a given memory less hypothesis for the classification task (might be useful classifier) which we do not have access to unless through query calls of inputs. Let $p_{h_0}$ denote the label distribution when we apply $h_0$ to source data and $q_{h_0}$ the counter part of target domain. Moreover, let $\wh p_{h_0},\wh q_{h_0}\in\Re_+^k$ denote their empirical approximation. 
For the label shift problem of interest, the anti-causal setting; we have
\begin{align}\label{eq:anti-causal}
    \D_p(\cdot|y)=\D_q(\cdot|y),~\forall y\in\Y
\end{align}
Furthermore, we require $\forall y\in \Y$, if $q(y)\geq 0$, then $p(y)\geq 0$. This is a reasonable setting since without any further prior knowledge, there is no way to properly reason about a class that does not exist in the source domain but appears in the target. Moreover, we need $h_0$ to be useful in some sense. For example if $h_0$ almost always output a fix class, then it does not capture any characteristics of the the data. Therefore, we are interested in the classifier which does not results in singularity in the spectrum of confusion matrix, i.e.
\begin{align*}
    C=\D_p(Y',Y)
\end{align*}
is full rank matrix where $Y':=h_0(X)$. If this matrix is singular, therefore class distributing is not identifiable under $h_0$. For example if two rows of $C$ are same, therefore there are two classes, $i$ and $j$ that $h_0$ assigns any true label identically to either $i$ or $j$ with the same probability which is a pathological setting. We define $\omega$ as the importance weight between these two domain $\omega_i=\frac{q(y=i)}{p(y=i)}=\frac{q_i}{p_i}$ and a notion of shift as $d(\D_q||\D_p)=d(q||p)=:\E_q\left[\omega_YY\right]=\sum_i^kq_i\frac{q_i}{p_i}$. We just look at class distribution since due to anti-causal setting, 
\begin{align*}
\frac{\D_q(X,y=i)}{\D_p(X,y=i)}=\frac{\D_q(X|y=i)q_i}{\D_p(X|y=i)p_i}=\frac{q(y=i)}{p(y=i)}
\end{align*}
We measure the shift by $d(\D_q||\D_p)$, which is equivalent to the exponent of second order Renyi divergence. Given a hypothesis class $\HH$, a loss function $l:\Y\times\Y\rightarrow [0,1]$ we define the expected loss of a classifier $h\in\HH$ as 
\begin{align*}
    L(h)=\E_{X,Y\sim\D_p}\left[\omega_Yl(Y,h(X))\right]=\E_{X,Y\sim\D_q}\left[l(Y,h(X))\right]
\end{align*}
Therefore, in order to find the classifier which generalize well in target set, we minimize the empirical weighed risk. 


==> Fanny-5-OSE.tex <==
\section{Online Label Shift Learning (\ose)}


\paragraph{Oracle approach: Weighting the training samples:}
A natural approach to correct for label shift is analogous to
weighting the samples by probability ratio in the covariate
shift setting.

Let us denote the marginal probability mass functions of $y$ for
$\disP, \disQ$ shorthand as $p, q: [k] \to [0,1]$ with $p(i) = \disP(Y
= i)$, and $q(i) = \disQ(Y
= i)$ for all $i \in [k]$, representable by vectors in $\Real_+^k$
which sum to one.
Given a hypothesis class $\HH$, a loss function $\loss:\Y\times\Y\rightarrow [0,1]$ our aim is to find the hypothesis $h\in\HH$ which minimizes
\begin{align*}
    \LossPop (h) =\E_{(X,Y)\sim\disQ}\left[\loss(Y,h(X))\right] = \E_{(X,Y)\sim\disP}\left[\weight(Y) \loss(Y,h(X))\right]
\end{align*}
where $\weight(i) = \frac{q(i)}{p(i)}$. In the usual finite sample
setting however, $\LossPop$ unknown and we are given samples $\{(x_j, y_j)\}_{j=1}^n$ from $\disP$ instead. If we are given the  We could then minimize the empirical
loss defined as
\begin{align*}
    \LossPop_n (h)=\frac{1}{n}\sum_{j=1}^n \weight(y_j)\loss(y_j,h(x_j))
\end{align*}
where $n$ is the number of available observations used to learn the
classifier $h$.  In reality however, $\weight$ is unknown as well,
so that we are effectively finding the minimizer
\begin{align}
  \label{eq:estimweightloss}
    \LossPop_n(h;\wh\weight)=\frac{1}{n}\sum_{j=1}^n\wh\weight(y_j)\loss(y_j,h(x_j))
\end{align}
where $\wh\weight$ are estimates of $\weight$.

We propose to use two-step procedure, given a set $\datap$ of $\np$ samples from
the source distribution $\disP$, we first divide the data set into two
sets where we use $(1-\beta)\np$ samples in set $\datapweight$ to
compute the estimate $\wh \weight$ and then the remaining $n= \beta
\np$ in the set $\datapclass$ to find the hypothesis which minimizes
the loss~\eqref{eq:estimweightloss}, i.e. $ \estweight = \argmin_{h\in \HH} \LossPop_n(h;\wh\weight)$.

In the following we describe how to estimate the
weights $\wh \weight$ and provide guarantees for the resulting
estimator $\estweight$.

\paragraph{Estimating weights while correcting for measurement error}

The following simple correlation between the label distributions $p,q$ was noted in~\citep{lipton2018detecting}: for a fixed hypothesis, it holds that for all $i,j\in\Y$, we have
\begin{align*}
    q_{h}(Y=i)&=\sum_j \disQ(h(X)=i|Y=j)q(j)=\sum_j \disP(h(X)=i|Y=j)q(j)\\
    &=\sum_j \disP(h(X)=i,Y=j)\frac{q(j)}{p(j)}=\sum_j \disP(h(X)=i,Y=j)\weight_j
\end{align*}
which can equivalently be written in matrix vector form (by slight abuse of notation) as
\begin{align}\label{eq:linear-model}
    q_{h}= \confmat_h \weight
\end{align}
where $C_h$ is the confusion matrix, that is $[C_h]_{i,j} = \disP(h(X)
= i, Y = j)$ and $q_h$ is the vector
which represents the probability mass function.  In general, both
$q_h$ and $\confmat_h$ can only be estimated by the corresponding
finite sample averages $\wh q_h, \wh\confmat_h$.

In the paper~\citep{lipton2018detecting}, the authors simply use
plug-in estimators and minimize $\|\wh \confmat_h \weight - \wh q_h\|_2$
directly.  Although it is an optimal approach to solve a Gaussian noise model 
when $\confmat_h$ is known to be precise,
there is no theoretical justification to plug in a noisy
$\wh \confmat_h$. Furthermore, when there are very few samples, the
weight estimation will have high variance in which case it might
be better to avoid importance weighting altogether. 

Instead, we propose to use the following two-step procedure to compute
importance weights: Given a ``decent'' black box estimator $\bbe$, we
\begin{enumerate}
\item calculate the measurement error adjusted $\thetaint$ as described in Section~\ref{sec:correctest} for $\bbe$,
compute the regularized weight $\wh \weight = \allones + \lambda \thetaint$ where $\lambda$ depends on the sample size $(1-\beta)\np$ and
  \item compute the minimizer $\estweight$ of the loss $\Loss_n(h; \wh\weight)$ in the hypothesis class $\HH$ with respect to $h$ 
\end{enumerate}

In order to estimate the weights using the relationship in
equation~\eqref{eq:linear-model}, it is necessary to use some
prediction model, which we call $\bbe$, to begin with.  The choice of
the model determines the conditioning of solving both the oracle
population but also the finite sample version of
~\eqref{eq:linear-model}.  In the paper~\citep{lipton2018detecting},
it was assumed that $\bbe$ was a fixed a priori given black box
estimator which we have at our disposal and we will do the same.
Obviously in practice the black box estimator is not fixed and the
conditioning of $\confmat_{\bbe}$ determines estimation accuracy and
the computational complexity. We will further discuss the choice of an
appropriate innitial black box estimation model $\bbe$ for implementation purposes in the experimental section.


\subsection{Corrected estimate}
\label{sec:correctest}
Both the design matrix and label distribution $\confmat_{\bbe},
q_{\bbe}$ on the target for black box hypthesis $\bbe$ are unknown and
we are only given finite sample estimates $\wh \confmat_{\bbe}, \wh
q_{\bbe}$.
under the Gaussian assumption it is standard to use the
total least squares approach which requires a single value
decomposition. 
\fycomment{Provide some explanation why we are not
  doing it here}
We use a different approach which targets the same type of measurement
errors.  Note that in what follows all empirical and population
confusion matrices as well as label distributions are defined with
respect to the hypothesis $h = \bbe$.  For notational simplicity, we
thus drop the subscript $\bbe$ in the in what follows.

In the unweighted case $\weight = \allones$, and thus the amount of weight shift
is captured in $\theta = \weight - \allones$. The reparameterized linear model~\eqref{eq:linear-model} with respect to $\theta$ then reads
\begin{equation*}
   b:= q - \confmat \allones = \confmat \theta
\end{equation*}
with corresponding finite sample quantity $\wh b = \wh q - \wh \confmat \allones$. 
When $\wh \confmat$ is near singular, the estimation of $\theta$ becomes unstable.
Furthermore, small values in the true weight $\weight$ result in large variances.
We address this problem by adding a regularizing $\ell_2$ penalty term to the usual loss
and thus push the amount of shift towards $0$, a method that has been proposed in \citep{pires2012statistical}.
In particular, we compute
\begin{equation}
  \label{eq:weightint}
  \thetaint = \argmin_{\thetaint_\rho \in \{2^{i+1}\Delta_C \Delta_b, i\in \NN\}} \|\wh \confmat \thetaint_{\rho}- \wh b\|_2 + 3 \Delta_C \|\thetaint_{\rho}\|_2
\end{equation}
%% We consider the weight estimate 
%% \begin{equation}
%%   \label{eq:weightint}
%%   \weightint = \argmin_{\weightint_\rho \in \{2^{i+1}\Delta_C \Delta_q, i\in \NN\}} \|\wh \confmat \weightint_{\rho}- \wh q\|_2 + 3 \Delta_C \|\weightint_{\rho}-1\|_2
%% \end{equation}
where $\thetaint_\rho$ is defined by 
\begin{equation}
  \thetaint_\rho = \argmin_{\theta'} \| \wh\confmat \theta' - \wh b\|^2_2  + \rho \| \theta'\|_2.
\end{equation}

Here, $\Delta_C, \Delta_b$ are parameters which will then be chosen to
be high probability upper bounds for $\|\wh \confmat - \confmat\|_2$
and $\|\wh b- b\|_2$ respectively.  Let $\sigma_{\min}$ be the minimum
singular value of the true confusion matrix $\confmat$.  For the
estimate $\thetaint$ we have the following upper bound

\begin{lemma}
\label{lem:weightest}
For $\thetaint$ as defined in equation~\eqref{eq:weightint}, we have with probability at least $1-\delta$ that
\begin{align*}
  \|\thetaint-\theta\|_2\leq
  O \left( \frac{1}{\sigma_{min}}\big( (\|\theta\|_2 + 1)\sqrt{\frac{\log (k/\delta)}{(1-\beta)\np}} + \sqrt{\frac{\log(1/\delta)}{m}}\big)\right)
  %% \frac{1}{\sigma_{min}}\left(\frac{2\|\weight\|_2}{(1-\beta)\np}+\|\weight\|_2\sqrt{\frac{18\log\left(4k/\delta\right)}{(1-\beta)\np}}+\sqrt{\frac{36\log\left(2/\delta\right)}{m}}\right)
\end{align*}
where $\delta < 0.5$.
\end{lemma}
\fycomment{I summarized the $\log k$ and $\|\theta\|_2$ term ...}

A couple of remarks are in order at this point.
First of all, notice that the upper bound in Lemma~\ref{lem:weightest} includes $\sigma_{\min}(\confmat)$ as a parameter, apart from the norm of the true weight shift $\theta$. Recall that these quantities are all heavily dependent on the
black box estimator $\bbe$ that we are given a priori. In particular, if $h$ is an ideal estimator, and the source
set is balanced, $\confmat$ is the unit matrix with $\sigma_{\min}=1/k$. In contrast, when the model $\bbe$ is uncertain, the singular value $\sigma_{\min}$ is close to zero.

\fycomment{Discuss the choice of $\rho$ in real implementations...}
%% \begin{theorem}[Generalization bound for $\est_{\weightint}$]
%% \label{thm:genbound}
%% Given a finite hypothesis class $\HH$ with cardinally of $|\HH|$, $n$ sample from the source data set, $m$ sample input from target set results in the following generalization bound.
%% \begin{align}\label{eq:Lhatwhat}
%%   |L(\est_{\weightint})-L(h^*)|
%%   &\leq
%%   2 \Rade_n(\G) + \dismaxpq \sqrt{\frac{\log 2/\delta}{n}} \\
%%   &+ O \left( \frac{1}{\sigma_{min}}\big( \|\weight\|_2 \sqrt{\frac{\log (k/\delta)}{(1-\beta)\np}} + \sqrt{\frac{\log(1/\delta)}{m}}\big)\right)\nonumber

%% \end{align}
%% with probability at least $1-\delta$ where $\delta\leq 0.5$.
%% \end{theorem}

\subsection{Regularized estimator and generalization bound}
When the number of samples in the target set or the shift is very low,
for example in the scenario where the estimated weights might be too
uncertain to be applied.  We therefore propose a regularized estimator
to correct for label shift in the anti-causal learning which is defined as follows
\begin{equation}
%  \wh \weight = (1 - \lambda)\textbf{1} + \lambda \weightint.
    \wh \weight = \textbf{1} + \lambda \thetaint.
\end{equation}
Intuitively, by rewriting $\wh\weight =(1 - \lambda)\textbf{1} + \lambda (\allones + \thetaint)$, 
we see that $\lambda$ should be closer to $1$ the more reason there is to belief that
$\allones + \thetaint$ is in fact the true weight. 

Notice that $\wh \weight$ implicitly depends on $\lambda, \beta$.  If
we now use $\wh \weight$ to compute $\estweight$ with $n = \beta \np$,
we can bound the generalization error using two key quantities
\begin{equation}
  \dispq := \E_{\disP} \weight^2(Y) = \sum_{i=1}^k q(i)\frac{q(i)}{p(i)} \qquad \text{and } \qquad \dismaxpq = \sup_i \frac{q(i)}{p(i)}.
\end{equation}
and the typical Rademacher complexity measure for the size of a
hypothesis class $\Rade_n(\G) := \sup_{h\in\HH} \frac{1}{n}
\sum_{i=1}^n \epsilon_i \weight(y_i) \loss(x_i, h(y_i))$.


\begin{theorem}[Generalization bound for $\estweight$]
\label{thm:genbound}
Given a finite hypothesis class $\HH$ with cardinally of $|\HH|$, $n$
sample from the source data set, $m$ sample input from target set
results in the following generalization bound.
\begin{align}\label{eq:Lhatwhat}
  |L(\estweight)-L(h^*)|&\leq
  2 \Rade_n(\G) + \dismaxpq \sqrt{\frac{\log 2/\delta}{n}}+ \left(1-\lambda\right)\|\theta\|_2\\
  %% \frac{2 \dismaxpq \left( \log(|\HH|)+\log(\frac{3}{\delta})\right)}{3\beta \np}+\sqrt{\frac{8\left(\dispq\right)\left(\log(|\HH|)+\log(\frac{3}{\delta})\right)}{\beta \np}}\nonumber\\
    %% &+\frac{\lambda}{\sigma_{min}}\Bigg(\frac{2\|\theta\|_2\log\left(3k/\delta\right)}{(1-\beta)\np} \\
  %% &\quad\quad\quad~~+\|\theta\|_2\sqrt{\frac{18\log\left(6k/\delta\right)}{(1-\beta)\np}}+\sqrt{\frac{36\log\left(3/\delta\right)}{(1-\beta)\np}}+\sqrt{\frac{36\log\left(3/\delta\right)}{m}}\Bigg)
  &+\frac{\lambda}{\sigma_{\min}} O\Bigg((\|\theta\|_2 + 1)\sqrt{\frac{18\log\left(6k/\delta\right)}{(1-\beta)\np}}
  %+\sqrt{\frac{36\log\left(3/\delta\right)}{(1-\beta)\np}}
  +\sqrt{\frac{36\log\left(3/\delta\right)}{m}}\Bigg) \nonumber
\end{align}
with probability at least $1-\delta$ where $\delta\leq 0.5$.
\end{theorem}

The proof can be found in Section~\ref{proof:genbound}.

\fycomment{re Kamyar: yeah we can get a better dependence on $p,q$ (that is $\dismaxpq$ for finite
  hypothesis class with union bound and Bernstein $\dispq$ but 1. it's not
  the main point so I'm glossing over it here, 2. we usually don't have finite classes in application so why show it for that particular case}
 \Kamyar{Please bring back the d and the discussion I had on it. The same union bound used for finite function class aslo holds for Rademacher. Also, other stuff in the draft I wrote, please bring those also back. No need to have all of them in the main text, but  have them all in the apx.}
 \fycomment{I'm open to discussion, but please be more specific what exactly you are missing, see email. Your original writing is untouched in the tex files (I only commented them out) you may add back whatever you like as long as notation & flow stay consistent and no unnecessary lemmas/steps are added.}

How large $\Rade_n(\G)$ is determined by the function class and
depends on the structure of $\HH$ and the loss $\loss$. For example
for the $0/1$ loss, the Rademacher complexity is upper bounded by
$\Rade_n(\G) \leq \dismaxpq \sqrt{\frac{\nu \log n}{n}}$ where $\nu$ is the
VC dimension of $\G(\loss, \HH)$ so that we have
\begin{equation*}
  \sup_{h\in\HH} |\Loss_n(h) - \Loss(h)| \leq  \dismaxpq \sqrt{ \frac{\nu\log \frac{2(n+1)}{\delta}}{n}} 
\end{equation*}

\fycomment{Discuss how $\weight$ comes in, something like Kamyar's text below}
To parse this bound, as we can see, it no more depends on $\|\omega\|_2$ rather to $\|\textbf{1}-\weight\|_2$ which goes to zero in low shift setting, also the regularization in Eq.~\ref{eq:theta-rho} and \ref{eq:thetahat-optimal} tend to make the importance weights close to no shift setting. Another super interesting characteristics of this bound is in its dependency on cardinality of label space, $k$. This dependency appears as $\log(k)$ which allows for combinatorially big classification tasks. It means for multi-label classification, e.g. each person can have multiple diseases at once, while we should be careful about possible growth of $\|\theta\|_2$. 

\fycomment{Discuss role of $\beta,\lambda$, something like Kamyar's text below}
Now there are two main question left. First is the choice of $\beta$ which needs to be chosen a priori from the set $\B$ (before applying the final classifier on the target domain). Second one is the case when the number samples in the source and target are fairly small, and also the shift induced by $\theta$ is big or small.

In order to use Theorem~\ref{thm:genbound} in practice, with ideal
$\lambda, \beta$, we need to assume some a priori knowledge of an
upper bound $\thetamax$ of the possible shifts we might encounter, i.e.
\begin{equation}
  \label{eq:maxweight}
  \|\theta\|_2 \leq \thetamax.
\end{equation}
and we consider the following cruder bound instead for 
practical implementation
\begin{align}\label{eq:Lhatwhatmax}
  |L(\estweight)-L(h^*)|&\leq
  2 \Rade_n(\G) + \dismaxpq \sqrt{\frac{\log 2/\delta}{n}}+ \left(1-\lambda\right)\thetamax\\
  %% \frac{2 \dismaxpq \left( \log(|\HH|)+\log(\frac{3}{\delta})\right)}{3\beta \np}+\sqrt{\frac{8\left(\dispq\right)\left(\log(|\HH|)+\log(\frac{3}{\delta})\right)}{\beta \np}}\nonumber\\
    %% &+\frac{\lambda}{\sigma_{min}}\Bigg(\frac{2\|\theta\|_2\log\left(3k/\delta\right)}{(1-\beta)\np} \\
  %% &\quad\quad\quad~~+\|\theta\|_2\sqrt{\frac{18\log\left(6k/\delta\right)}{(1-\beta)\np}}+\sqrt{\frac{36\log\left(3/\delta\right)}{(1-\beta)\np}}+\sqrt{\frac{36\log\left(3/\delta\right)}{m}}\Bigg)
  &+\frac{\lambda}{\sigma_{\min}} O\Bigg(\thetamax \sqrt{\frac{\log\left(k/\delta\right)}{(1-\beta)\np}}
  %+\sqrt{\frac{36\log\left(3/\delta\right)}{(1-\beta)\np}}
  +\sqrt{\frac{\log\left(3/\delta\right)}{m}}\Bigg) \nonumber
\end{align}


Intuitively, when the number of samples in the target domain, $m$, is low, the last term in the Eq.~\ref{eq:Lhatwhatmax} grows. Consider the case where $\thetamax$ is small, then we intuitively prefer to do not use our estimated $\wh \weight$ and just use the a good classifier trained directly on the source data to use against target data. On other hand, consider the case where $\thetamax$ is large. In this setting, since the shift is big, even a signal sample from the target domain is highly helpful and informative to enhance the classifier by far. In this setting we like to fully use the estimated $\wh\weight$ to train the suitable classifier against target set. There are setting in between that we might like to regularize the estimated importance weights $\wh \weight$ a bit toward shift setting. We introduce $\lambda$- shifted importance weight as $\wh\weight=\textbf{1}+\lambda \wh \theta$, with $0\leq\lambda\leq 1$. For this case, $\lambda=0$ means regularize all the way to no shift setting, while $\lambda=1$ means to keep the weights as they are and no further regularization. We consider the setting with a set of possible $\lambda$'s from a finite set of $\Lambda$ which we can chose $\lambda$ a priori. Therefore, putting these two components of the generalization together we get;


A simple manipulation shows that the optimal $\lambda$ is either zero or one. Since the bound is constructed for worst case scenario, in order to choose a useful $\lambda$ for practice, we follow the Bayesian interpretation of this bound. In practice we do not have $\theta_{\max}$ but just a belief of it and also the concentration bounds also follow  Bayesian posteriors which results in $\lambda$ between zero and one.
Then the useful lambda has an interesting behaviour with respect to the detail parameters, i.e. $\lambda^*\approx\max\lbrace 0,\min\lbrace \thetamax-\mathcal{O}(\thetamax/\sqrt{n})-\mathcal{O}(1/\sqrt{n})-\mathcal{O}(1/\sqrt{m}),1\rbrace\rbrace$.%\footnote{Since we have a linear program on the solution is either zero or one but in practice we do not have $\theta_{\max}$ but just a belief of it and also the concentration bounds can also become Bayesian which results in $\lambda$ between zero and one.}

\subsection{Regularized estimator for the streaming setting}

Consider a setting where we send a group of volunteers to a new
country with new disease distribution of dangerous disease for at most
$T$ time step. In this case we do not like to wait to collect enough
samples in order to train a classifier. We are interested in updating
our model more often, even maybe after visiting each new patient.
Note that the regularization enables us to update our classifier $h$
in settings where we only have few samples in the target set, e.g. when we
have only observed symptoms from very few patients in a different
country.

%% \ose estimates the importance weights $\weight$ in a principled way by solving multiple small convex problems Then uses the estimated weight to train a classifier. 
We thus propose to use the following algorithm in the streaming
setting when at time $t$ we have acquired $t$ unlabeled samples from
the target set. The key is that we can choose both $\beta^\star, \lambda^\star$ at any
time step depending on $t$, described in the algorithm below.

\input{algorithm}
\fycomment{the $\lambda^\star$ in the algorithm is probably not the actual minimization (since that would be $0,1$) but the heuristic you described above...}

Note: Obviously it is very costly to compute both $\lambda^\star, \beta^\star$ and recompute the classifier after each new sample is obtained. We want to emphasize that the step in the loop can be skipped as desired and as the budget allows. The accuracy guarantees given in  Corollary~\ref{cor:streaming} still hold.


The generalization bound for $\estweight$ in this setting directly follows from
Theorem~\ref{thm:genbound} and the union bound.
\begin{corollary}[Generalization Bound for the streaming setting]
\label{cor:streaming}
For the estimator $\estweight^t$ in Algorithm~\ref{alg:ose} after running $\ose$ for $t$ time steps 
we obtain the following upper bound on the generalization error
%   Given a finite hypothesis class $\HH$ with cardinally of $|\HH|$,
%   $\np$ samples from the source data set, splitting set $\B$,
%   regularization set $\Lambda$, after $t$ time steps of running \ose, and $t$
%   observations from the target domain, we have
\begin{align}\label{eq:finalbound}
  |L(\estweight^t)-L(h^*)|&\leq
  2 \Rade_n(\G) + \dismaxpq \sqrt{\frac{\log 2t/\delta}{n}}+ \left(1-\lambda\right)\|\theta\|_2\\
  %% \frac{2 \dismaxpq \left( \log(|\HH|)+\log(\frac{3}{\delta})\right)}{3\beta \np}+\sqrt{\frac{8\left(\dispq\right)\left(\log(|\HH|)+\log(\frac{3}{\delta})\right)}{\beta \np}}\nonumber\\
    %% &+\frac{\lambda}{\sigma_{min}}\Bigg(\frac{2\|\theta\|_2\log\left(3k/\delta\right)}{(1-\beta)\np} \\
  %% &\quad\quad\quad~~+\|\theta\|_2\sqrt{\frac{18\log\left(6k/\delta\right)}{(1-\beta)\np}}+\sqrt{\frac{36\log\left(3/\delta\right)}{(1-\beta)\np}}+\sqrt{\frac{36\log\left(3/\delta\right)}{m}}\Bigg)
  &+\frac{\lambda}{\sigma_{\min}} O\Bigg((\|\theta\|_2 + 1)\sqrt{\frac{\log\left(kt/\delta\right)}{(1-\beta)\np}}
  %+\sqrt{\frac{36\log\left(3/\delta\right)}{(1-\beta)\np}}
  +\sqrt{\frac{\log\left(t/\delta\right)}{t}}\Bigg) \nonumber
\end{align}
% \begin{align}\label{eq:finalbound}
%     |L(\estweight^t)-L(h^*)|&\leq \frac{2 \dismaxpq \left( \log(|\HH|t)+\log(\frac{3}{\delta})\right)}{3\beta \np}+\sqrt{\frac{8\left(\dispq\right)\left(\log(|\HH|t)+\log(\frac{3}{\delta})\right)}{\beta \np}}\nonumber\\
%     &+ \left(1-\lambda\right)\|\theta\|_2+\frac{\lambda}{\sigma_{min}}\Bigg(\frac{2\|\theta\|_2\log\left(3kt/\delta\right)}{(1-\beta)\np}\\
% &\quad\quad\quad~~+\|\theta\|_2\sqrt{\frac{18\log\left(6kt/\delta\right)}{(1-\beta)\np}}+\sqrt{\frac{36\log\left(3t/\delta\right)}{(1-\beta)\np}}+\sqrt{\frac{36\log\left(3t/\delta\right)}{t}}\Bigg)
% \end{align}
with probability at least $1-\delta$ when $\delta<0.5$.
\end{corollary}

%Proof. in Theorem.~\ref{thm:gen-reparam-opt-online}
% \fycomment{something is still weird - we only use $t$ samples at each step, what's that $m$ doing in the bound}\Kamyar{Fixed}

%% In the next section we give theoretical guarantees for our weighted procedure for general hypothesis classes. By bounding the difference true and estimated weights, we obtain upper bounds for the excess risk for our weighted estimator.

%% We theoretically analyzed an efficient way to estimate the importance weights. We empirically investigate the power of our estimator under verity of label shifts and compared it to the previous work.





==> Old/5-Generalization.tex <==
\section{Generalization under Label Shift}
In this section, we develop a generalization theory for the label shift problem of interest. Under assumption in Eq.\ref{eq:anti-causal}, we have, $~\forall i,j\in\Y$
\begin{align*}
    \D_q(Y'=i|Y=j)&=\int_{x\in\X}\D_q(h_0(x)=i|X=x)\D_q(X=x|Y=j)dx\\
    &=\int_{x\in\X}\D_p(h_0(x)=i|X=x)\D_p(X=x|Y=j)dx=\D_p(Y'=i,Y=j).
\end{align*}

Therefore, with an elementary manipulation, we get;$\forall i,j\in\Y$
\begin{align*}
    q_{h_0}(Y=i)&=\sum_j \D_q(Y'=i|Y=j)q(j)=\sum_j \D_p(Y'=i|Y=j)q(j)\\
    &=\sum_j \D_p(Y'=i,Y=j)\frac{q(j)}{p(j)}=\sum_j \D_p(Y'=i,Y=j)\omega_j
\end{align*}
Therefore, deploying the definition of the confusion matrix we have;
\begin{align}\label{eq:linear-model}
    q_{h_0}=C\omega
\end{align}
Therefore, if we have $C$ and $q_{h_0}$, we also have the vector of importance weights. But in practice we just have access to estimation of $q_{h_0}$, i.e. $\wh q_{h_0}$ and C, i.e. $\wh C$. In this section we show how to use part of source data to estimate the importance weights and, then deploy the estimated weights to learn the desire classifier. In other works, we randomly split the source set into two distinct sets of size $\lbrace(1-\beta)n,\beta n\rbrace$, $D_p^\beta$ and $D_p^{1-\beta}$ as the set to learn the importance weight and the set to learn the proper classifier for the target set while $\beta$ is chosen from a finite set of $\B$ with cardinality $|\B|$. It is worth noting that the number of possible $\beta$ is upper bounded by $n+1$ while empirically we might be interested to just consider a small subset of $\beta$ which is set $\B$. Therefore, the emperical loss when the importance weights are givens is
\begin{align*}
    \wh L(h)=\frac{1}{\beta n}\sum_{(x_i,y_i)\in D_p }\omega_{y_i}l(y_i,h(X_i))
\end{align*}
where we are interested in $L(h)-\wh L(h)$ as well as excess risk $L(\wh h)-\wh L(h^*)$ where $h^*:=\arg\min_{h\in\HH}L(h)$ is the hypothesis with minimum expected loss, and $\wh h=\arg\min_{h\in\HH}\wh L(h)$ is the empirical average loss minimizer. Afterward, when we have the estimated importance weighs, we are interested in 
\begin{align*}
    \wh L(h;\wh\omega)=\frac{1}{\beta n}\sum_{(x_i,y_i)\in D_p^\beta }\wh\omega_{y_i}l(y_i,h(X_i))
\end{align*}
where similarly we are interested in $L(h)- \wh L(h;\wh\omega)$ as well as excess risk $ \wh L(h;\wh\omega)- \wh L(h^*;\wh\omega)$ where now $\wh h_{\wh\omega}=\arg\min_{h\in\HH} \wh L(h;\wh\omega)$ is the empirical average loss minimizer. But before the generalization study, we investigate in estimating  $\omega$.

\paragraph{Measurement Error Models}
For the measurement error problem of, $q_{h_0}=C\omega$ where we have the noisy observation of both measurements $q_{h_0}$ and instrument, the measurement matrix, C we deploy Instrumental Variable Method. As mentioned before, we utilize $D_p^{1-\beta}$, $1-\beta$ portion of the source data to for estimation the importance weights. Moreover, we use the whole target set for this task. The detailed proof of the following statements are appeared in the Appendix, section.~\ref{sec:measuremnt}, Theorem.~\ref{thm:concentration-theta}, and Lemma.~\ref{lemma:concentration-theta}. 

\begin{lemma}[Concentration of measurement matrix $\wh C$]
Given the samples in data set $D_p^{1-\beta}$ and classifier $h_0$, we approximate $C$ through its empirical average of $\wh C=\frac{1}{(1-\beta)n}\sum_{(x_i,y_i)\in D_p}\left[e_{h_0(x_i)}e_{y_i}^{\top}\right]$ where $e_i$ is one-hot-encoding of index $i$. then 
\begin{align*}
    \|\wh C-C\|_2\leq \Delta_C:=\frac{2\log\left(2k/\delta\right)}{3(1-\beta)n}+\sqrt{\frac{2\log\left(2k/\delta\right)}{(1-\beta)n}}
\end{align*}
with probability at least $(1-\delta)$. Proof. Lemma.~\ref{lemma:C}
\end{lemma}
Furthermore,
\begin{lemma}[Concentration of measurements] 
Given the samples in data set $D_q$ and classifier $h_0$, we approximate $q_{h_0}$ through its empirical estimator of $\wh q_{h_0}=\frac{1}{m}\sum_i^me_{h_0(x_i)}$, then
\begin{align*}
    \|\wh q_{h_0}-q_{h_0}\|\leq\Delta_q:= \frac{1}{\sqrt{m}}+\sqrt{\frac{\log\left(1/\delta\right)}{m}}
\end{align*}
with probability at least $1-\delta$. Proof. Lemma.~\ref{lemma:b}
\end{lemma}
In the Appendix, specially in Theorem.~\ref{thm:concentration-theta}, we show that if we solve this measurement problem as it is, we get a unpleasant dependency of $\|\omega\|_2$ in the generalization bound. This parameter, does not vanish even in no shift setting, where $\omega=\textbf{1}$, a vector of all ones. We introduce a trick in change of variable in order to remove the unpleasant effect. 
\begin{align*}
    \omega:=\textbf{1}+\theta,\quad \wh\omega:= \textbf{1}+\wh\theta
\end{align*}
which results in the following problem: $q_{h_0}-p_{h_0}=C\theta$. Similar argument in Lemma \ref{lemma:b} also holds for concentration of $\wh p_{h_0}$, with probability at least $1-\delta$
\begin{align*}
    \|\wh p_{h_0}-p_{h_0}\|\leq\Delta_p:= \frac{1}{\sqrt{(1-\beta)n}}+\sqrt{\frac{\log\left(1/\delta\right)}{(1-\beta)n}}
\end{align*}
Now, since we have the concentration of the $C,q_{h_0},p_{h_0}$, we follow the following hyper parameter free procedure in order to find the desire $\wh\theta$ and therefore, the desire $\wh\omega$. Give a set of regularization parameter $\rho\in\lbrace 2^{i+1}\Delta_C\left(\Delta_q+\Delta_p\right)~, ~i\in\mathbb{N}\rbrace$ regularization $\rho$,
\begin{align}\label{eq:theta-rho}
\wh \theta_\rho:=\arg\min_\theta\lbrace\|\wh C\theta'-\wh q_{h_0}+\wh p_{h_0}\|_2^2+\rho\|\theta'\|_2\rbrace    
\end{align}
and
\begin{align}\label{eq:thetahat-optimal}
\wh\theta:=\arg\min_{\wh \theta\rho:\rho\in\lbrace 2^{i+1}\Delta_C\Delta_b~, ~i\in\mathbb{N}\rbrace}\lbrace\|\wh C\wh\theta_\rho-\wh q_{h_0}+\wh p_{h_0}\|_2+3\Delta_C\|\wh\theta_\rho\|_2\rbrace.    
\end{align}
Obviously, for practical implementation of this algorithm, we do not try all possible $\rho$ but a finite set of them. This procedure gives us $\wh\theta$ which satisfies the following;
\begin{align}\label{eq:theta-error}
\|\wh\theta-\theta\|_2\leq \frac{1}{\sigma_{min}}\left(\frac{2\|\theta\|_2\log\left(3k/\delta\right)}{(1-\beta)n}+\|\theta\|_2\sqrt{\frac{18\log\left(6k/\delta\right)}{(1-\beta)n}}+\sqrt{\frac{36\log\left(3/\delta\right)}{(1-\beta)n}}+\sqrt{\frac{36\log\left(3/\delta\right)}{m}}\right)
\end{align}
with probability at least $1-\delta$ for $\delta\leq 0.5$, where $\sigma_{min}$ is smallest singular value of the confusion matrix. The proof of this inequality is described in full detail in Lemma.\ref{lemma:concentration-theta}.
To parse this bound, as we can see, it no more depends on $\|\omega\|_2$ rather to $\|\theta\|_2$ which goes to zero in low shift setting, also the regularization in Eq.~\ref{eq:theta-rho} and \ref{eq:thetahat-optimal} tend to make the importance weights close to no shift setting. Another super interesting characteristics of this bound is in its dependency on cardinality of label space, $k$. This dependency appears as $\log(k)$ which allows for combinatorially big classification tasks. It means for multi-label classification, e.g. each person can have multiple disease at once, while we should be careful about possible growth of $\|\theta\|_2$. 

\textbf{Note:} The choice of $\|\theta'\|_2$ for regularization rather than the common practice $\|\theta'\|_2^2$ and total least square is important in label shift. Consider a common practice setting with big shift which results in a big $\|\theta\|_2$. In this case, the bell-like regularization of $\|\theta'\|_2^2$ over-regularizes the estimated weight, while the cone-like regularization of $\|\theta'\|_2$ regularizes the weights roughly independent of their magnitude. 
\paragraph{Generalization}
Since we have good estimator of the importance weights, now we are able to characterize the generalization property of $\wh h_{\wh\omega}=\arg\min_{h\in\HH} \wh L(h;\wh\omega)$. But before that, we characterize the generalizations property of $\wh h=\arg\min_{h\in\HH}\wh L(h)$. In the following, for sake of simplicity of notation, we consider the finite hypothesis class of $\HH$. Obviously, the analysis on the generalization theory appeared in this work is directly extendable to any other notion desire complexity, e.g. Rademacher Complexity, Shattering coefficient, VC dimension, or norm on the hypotheses class \citep{vapnik2013nature} since we just need these notions to complete our union bound step of generalization. Let's $d_\infty(q||p):=\frac{q_i}{p_i}$ as the $\ell_\infty$ norm of $\omega$, therefore,

\begin{lemma}[Generalization bound with known $\omega$] Given a finite hypothesis class $\HH$ with cardinally of $|\HH|$, $n$ sample from the source data set, and access to the importance weights $\omega$,
\begin{align*}
    |L(\wh h)-L(h^*)|\leq \frac{2d_\infty(q||p)\left(\log(|\HH|)+\log(\frac{2}{\delta})\right)}{3\beta n}+\sqrt{\frac{8\left(d(q||p)\right)\left(\log(|\HH|)+\log(\frac{2}{\delta})\right)}{\beta n}}
\end{align*}
with probability at least $1-\delta$. Proof in Theorem.~\ref{thm:finite-h}
\end{lemma}
For any desire notion of complexity, with a simple manipulation, we just need to replace $\log(|\HH|)$ with the complexity notion at hand. An interesting aspect of this bound is its dependency in $d_\infty(q||p)$. Even though this term can be big, but its effect goes down as $1/n$ rather than slower rate of $1/\sqrt{n}$. The next question, which is the main motivation of this work is the generalization for the case of unknown $\omega$. 

\begin{theorem}[Generalization bound with estimated $\wh \omega$]
Given a finite hypothesis class $\HH$ with cardinally of $|\HH|$, $n$ sample from the source data set, $m$ sample input from target set results in the following generalization bound.
\begin{align}\label{eq:Lhatwhat}
    |L(\wh h_{\wh\omega})-L(h^*)|&\leq \frac{2d_\infty(q||p)\left(\log(|\HH|)+\log(\frac{3}{\delta})\right)}{3\beta n}+\sqrt{\frac{8\left(d(q||p)\right)\left(\log(|\HH|)+\log(\frac{3}{\delta})\right)}{\beta n}}\nonumber\\
    &\left(1-\lambda\right)\|\theta\|_2+\frac{\lambda}{\sigma_{min}}\Bigg(\frac{2\|\theta\|_2\log\left(3k/\delta\right)}{(1-\beta)n}\nonumber\\
&\quad\quad\quad~~+\|\theta\|_2\sqrt{\frac{18\log\left(6k/\delta\right)}{(1-\beta)n}}+\sqrt{\frac{36\log\left(3/\delta\right)}{(1-\beta)n}}+\sqrt{\frac{36\log\left(3/\delta\right)}{m}}\Bigg)
\end{align}
with probability at least $1-\delta$ where $\delta\leq 0.5$ . Proof at Theorem.~\ref{thm:gen-reparam}
\end{theorem}
\paragraph{The choices of $\beta$ and regularization}
Now there are two main question left. First is the choice of $\beta$ which needs to be chosen a priori from the set $\B$ (before applying the final classifier on the target domain). Second one is the case when the number samples in the source and target are fairly small, and also the shift induced by $\theta$ is big or small. For the rest, we consider the case that of prior knowledge that $\|\theta\|_2\leq \|\theta_{\max}\|_2$. Intuitively, when the number of samples in the target domain, $m$, is low, the last term in the Eq.~\ref{eq:Lhatwhat} grows. Consider the case where $\|\theta_{\max}\|_2$ is small, then we intuitively prefer to do not use our estimated $\wh \omega$ and just use the a good classifier trained directly on the source data to use against target data. On other hand, consider the case where $\|\theta_{\max}\|_2$ is large. In this setting, since the shift is big, even a signal sample from the target domain is highly helpful and informative to enhance the classifier by far. In this setting we like to fully use the estimated $\wh\omega$ to train the suitable classifier against target set. There are setting in between that we might like to regularize the estimated importance weights $\wh \omega$ a bit toward shift setting. We introduce $\lambda$- shifted importance weight as $\wh\omega=\textbf{1}+\lambda \wh \theta$, with $0\leq\lambda\leq 1$. For this case, $\lambda=0$ means regularize all the way to no shift setting, while $\lambda=1$ means to keep the weights as they are and no further regularization. We consider the setting with a set of possible $\lambda$'s from a finite set of $\Lambda$ which we can chose $\lambda$ a priori. Therefore, putting these two components of the generalization together we get;



\begin{theorem}[Generalization Bound with optimal data ration and regularization]
Given a finite hypothesis class $\HH$ with cardinally of $|\HH|$, $n$ sample from the source data set, splitting set $\B$, regularization set $\Lambda$, $m$ sample input from target set, with $\wh\omega=\textbf{1}+\lambda\wh\theta$, we have
\begin{align*}
    |L(\wh h_{\wh\omega})&-L(h^*)|\leq\min_{\beta\in\B}\Bigg\{ \frac{2d_\infty\left(\log(|\HH|)+\log(\frac{3|\B|}{\delta})\right)}{3\beta n}+\sqrt{\frac{8\left(d_{\max}\right)\left(\log(|\HH|)+\log(\frac{|\B|3}{\delta})\right)}{\beta n}}\nonumber\\
    &\!\!\!\!\!\!\!\min_{\lambda_\in\Lambda}\Bigg\{\left(1-\lambda\right)\|\theta_{\max}\|_2+\frac{\lambda}{\sigma_{min}}\Bigg(\frac{2\|\theta_{\max}\|_2\log\left(3k|\B||\Lambda|/\delta\right)}{(1-\beta)n}\\
&~~\!\!\!\!\!\!\!+\|\theta_{\max}\|_2\sqrt{\frac{18\log\left(6k|\B||\Lambda|/\delta\right)}{(1-\beta)n}}+\sqrt{\frac{36\log\left(3|\B||\Lambda|/\delta\right)}{(1-\beta)n}}+\sqrt{\frac{36\log\left(3|\B||\Lambda|/\delta\right)}{m}}\Bigg)\Bigg\}\Bigg\}
\end{align*}
with probability at least $1-\delta$ where $d_\infty$ is prior knowledge on maximum possible $d_\infty(q||p)$ and $d_{\max}$ the prior knowledge on maximum possible $d(q||p)$. Proof in Theorem.~\ref{thm:gen-reparam-opt}
\end{theorem}

Given this theorem, we can see the role that both $\beta$ and $\lambda$ play in the bound. A simple manipulation shows that the optimal $\lambda$ has an interesting behaviour with respect to the detail parameters, i.e. $\lambda^*\approx \left[\theta_{\max}/(\theta_{\max}-\mathcal{O}(1/n)-\mathcal{O}(1/m))\right]_0^1$\footnote{Since we have a linear program on the solution is either zero or one but in practice we do not have $\theta_{\max}$ but just a belief of it and also the concentration bounds can also become Bayesian which results in $\lambda$ between zero and one.}

The last part of the theoretical analysis is the streaming setting. Consider a setting where we send a group of volunteers to a new country with new disease distribution of dangerous disease. In this case we do not like to wait to collect enough samples in order to train a classifier. We are interested in updating our model more often, even maybe after visiting each new patient.
\begin{theorem}[Generalization Bound for online setting]
Given a finite hypothesis class $\HH$ with cardinally of $|\HH|$, $n$ sample from the source data set, splitting set $\B$, regularization set $\Lambda$, $m$ sample input from target set, with $\wh\omega=\textbf{1}+\lambda\wh\theta$, at each time step $t$ with $t$ observation from the target domain, we have $\forall i:i\leq t i\in\N $
\begin{align}\label{eq:final-bound}
    |L(\wh h_{\wh\omega^i}^i)&-L(h^*)|\leq\min_{\beta\in\B}\Bigg\{ \frac{2d_\infty\left(\log(|\HH|)+\log(\frac{3t|\B|}{\delta})\right)}{3\beta n}+\sqrt{\frac{8\left(d_{\max}\right)\left(\log(|\HH|)+\log(\frac{t|\B|3}{\delta})\right)}{\beta n}}\nonumber\\
    \!\!\!\!\!\!\!&\min_{\lambda_\in\Lambda}\Bigg\{\left(1-\lambda\right)\|\theta_{\max}\|_2+\frac{\lambda}{\sigma_{min}}\Bigg(\frac{2\|\theta_{\max}\|_2\log\left(3kt|\B||\Lambda|/\delta\right)}{(1-\beta)n}\nonumber\\
&~~\!\!\!\!\!\!\!+\|\theta_{\max}\|_2\sqrt{\frac{18\log\left(6kt|\B||\Lambda|/\delta\right)}{(1-\beta)n}}+\sqrt{\frac{36\log\left(3t|\B||\Lambda|/\delta\right)}{(1-\beta)n}}+\sqrt{\frac{36\log\left(3t|\B||\Lambda|/\delta\right)}{m}}\Bigg)\Bigg\}\Bigg\}
\end{align}
with probability at least $1-\delta$ with $\delta<0.5$. Proof. in Theorem.~\ref{thm:gen-reparam-opt-online}
\end{theorem}

\textbf{Important Note:} It is clear that if the set $\B$ and $\Lambda$ are single member sets, then all the $\|\theta_{\max}\|_2$, $d_{\max}$ and $d_\infty$ reduce to $\|\theta\|_2$, $d(q||p)$ and $d_\infty(q||p)$, we do not need to have prior knowledge. Moreover, the condition $\delta<0.5$ is there to remover some small terms in the bound, otherwise there is not need for them. 












==> Old/Concentrations.tex <==
\section{Measurement Error Models}\label{sec:measuremnt}
% \section{Errors-in-variables models/Measurement Error Models and Instrumental Variable Method}
Consider a measurement error problem with a specified positive definite matrix $M\in\Re^{k\times k}$, where the desire is to minimize $\Upsilon_M(\omega)$
\begin{align*}
    \Upsilon_M(\omega):=\|C\omega-b\|_M
\end{align*}
with the optimum at $\omega^*:=\arg\min  \Upsilon_M(\omega):=\arg\min \|C\omega-b\|_M$, $C\in\Re^{k\times k}$, and $b,\omega\in\Re^k$. Furthermore, consider the case that the problem is realizable and $\omega^*$ results in zero loss of $\Upsilon_M(\omega^*)=0$. Moreover, as followed for total least square problems, we have access to the noisy observation of measurement matrix $\wh C$, and noisy measurements of $\wh b$. Consider the following concentrations of the observations;
\begin{equation}
    \Delta C := \|C-\wh C\|_{\alpha,M}=\sup_{x\neq 0}\frac{\|\left(C-\wh C\right)x\|_M}{\|x\|_\alpha} ~~\textit{and},~~ \Delta b := \|b-\wh b\|_M,
\end{equation}
for some alpha. 
In the problem of interest in this work, we have statistical estimate of $C$, and $b$ while, as usual concentration inequalities, given $N$ sample, with high probability at least $1-\delta$, we get $\Delta C$ and  $\Delta b$ concentrate around zero under some proper mean. Consider the empirical loss of 
% we get $\Delta C\leq \xi_N^A\xi^C_\delta$ and  $\Delta b\leq \xi_N^b\xi^b_\delta$ where the mentioned decoupling of $\xi_N$ and $\xi_\delta$ comes from usual form of confidence bounds and we have $\xi_N=\mathcal{O}\left(\sqrt{1/N}\right)$ and $\xi_\delta=\mathcal{O}\left(\sqrt{log\left(\delta\right)}\right)$. Consider the empirical loss of 
\begin{align}\label{eq:total-least}
    \wh\Upsilon_M(\omega'):=\|\wh C\omega'-\wh b\|_M
\end{align}
and for a given regularization $\rho$,
\begin{align*}
\wh \omega_\rho:=\arg\min_\omega\lbrace\wh\Upsilon_M(\omega')^2+\rho\|\omega'\|_\alpha\rbrace    
\end{align*}
and
\begin{align}\label{eq:thetahat}
\wh\omega:=\arg\min_{\wh \omega_\rho:\rho\in\lbrace 2^{i+1}\Delta_C\Delta_b~, ~i\in\mathbb{N}\rbrace}\lbrace\wh\Upsilon_M(\wh\omega_\rho)+3\Delta_C\|\wh\omega_\rho\|_\alpha\rbrace.    
\end{align}

\begin{theorem}[Thm.~3.7 in \citep{pires2012statistical}]
For the problem in Eq.~\ref{eq:total-least}, if with probability at least $1-\delta$, $\Delta C\leq \Delta_C$ and $\Delta b\leq \Delta_b$ hold simultaneously, then
\begin{align}\label{eq:upperUpsilon}
\Upsilon_M(\wh\omega)\leq \inf_{\omega'}\lbrace \Upsilon_M(\omega')+3\Delta_C\|\omega'\|_\alpha\rbrace+3\Delta_b
\end{align}
\end{theorem}

\begin{theorem}[Concentration of $\wh \omega$]\label{thm:concentration-theta}
For the inverse problem in \ose Eq.~\ref{eq:total-least} where $C$ and $\wh C$ are confusion matrix and its estimate, while $b=q_{h_0}$ and $\wh b=\wh q_{h_0}$, if the $\wh\omega$, as the solution to Eq.~\ref{eq:thetahat} is considered, for $\alpha=2$ and $M=I$, we have
\begin{align*}
\|\wh\omega-\omega\|_2\leq \frac{1}{\sigma_{min}}\left(\frac{2\|\omega\|_2}{(1-\beta)n}+\|\omega\|_2\sqrt{\frac{18\log\left(4k/\delta\right)}{(1-\beta)n}}+\sqrt{\frac{36\log\left(2/\delta\right)}{m}}\right)
\end{align*}
with probablity at least $1-\delta$ for $\delta\leq 0.5$.
\end{theorem}
\begin{proof*}[ Thm.~\ref{thm:concentration-theta}]
We first analyze the solution possible solutions to the infimum optimization problem in the Eq.~\ref{eq:upperUpsilon}. For simplicity and due to realizable property of the problem we have;
\begin{align*}
    \inf_{\omega'}\lbrace \Upsilon_M(\omega')+3\Delta_C\|\omega'\|_2\rbrace=\inf_{\omega'}\lbrace \|C\omega'-b\|_M+3\Delta_C\|\omega'\|_2\rbrace\leq\lbrace \|C\omega'-b\|_M+3\Delta_C\|\omega'\|_2\rbrace\Big|_{\omega'=\omega}
\end{align*}
We bring the more detailed analysis of this optimization in Lemma \ref{lemma:inf}. Since for any $M$,  $\|A\omega-b\|_M=0$ therefore
\begin{align*}
    \inf_{\omega'}\lbrace \Upsilon_M(\omega')+3\Delta_C\|\omega'\|_2\rbrace\leq 3\Delta_C\|\omega\|_2
\end{align*}
as a consequence,
\begin{align*}
    \Upsilon_I(\wh\omega)=\|C\wh\omega-b\|_2=\|C\wh\omega-C\omega\|_2=\|C\left(\wh\omega-\omega\right)\|_2\leq 3\Delta_C\|\omega^*\|_2+3\Delta_b
\end{align*}
If we consider an SVD of $C=UDV^\top$, then we have $\|C\left(\wh\omega-\omega\right)\|_2=\|UDV^\top\left(\wh\omega-\omega\right)\|_2=\|DV^\top\left(\wh\omega-\omega\right)\|_2$ and since;
\begin{align*}
    \|DV^\top\left(\wh\omega-\omega\right)\|_2&=\sqrt{\sum_i\sigma_i^2V_i^\top\left(\wh\omega-\omega^*\right)}\geq \sqrt{\sum_i\sigma_{\min}^2V_i^\top\left(\wh\omega-\omega\right)}\\
    &=\sigma_{min}\|V^\top\left(\wh\omega-\omega\right)\|=\sigma_{min}\|\wh\omega-\omega\|
\end{align*}
therefore
\begin{align*}
\|\wh\omega-\omega\|_2\leq \frac{1}{\sigma_{min}}\left(3\Delta_C\|\omega\|_2+3\Delta_b\right)
\end{align*}

In the \ose problem, we have the noisy estimate of confusion matrix $C$ as $\wh C$, and estimate of $q_{h_0}$, as $\wh q_{h_0}$. By plugging in $b=q_{h_0}$ and $\wh b=\wh q_{h_0}$ and Lemma.~\ref{lemma:C} for concentration of $C$ and Lemma.~\ref{lemma:b} for concentration of $q_{h_0}$ we have
\begin{align*}
\|\wh\omega-\omega\|_2\leq \frac{1}{\sigma_{min}}\left(\frac{2\|\omega\|_2\log\left(2k/\delta\right)}{(1-\beta)n}+\|\omega\|_2\sqrt{\frac{18\log\left(4k/\delta\right)}{(1-\beta)n}}+\frac{3}{\sqrt{m}}+\sqrt{\frac{9\log\left(2/\delta\right)}{m}}\right)
\end{align*}
with probability at least $1-\delta$. If $\delta\leq 0.5$ then
\begin{align*}
\|\wh\omega-\omega\|_2\leq \frac{1}{\sigma_{min}}\left(\frac{2\|\omega\|_2\log\left(2k/\delta\right)}{(1-\beta)n}+\|\omega\|_2\sqrt{\frac{18\log\left(4k/\delta\right)}{(1-\beta)n}}+\sqrt{\frac{36\log\left(2/\delta\right)}{m}}\right)
\end{align*}
which is the statement of the theorem.~\ref{thm:concentration-theta}.
\end{proof*}



\begin{lemma}\label{lemma:inf}
The solution to the infimum optimization problem in the Eq.~\ref{eq:upperUpsilon}, $\wt\omega$
\begin{align*}
    \wt\omega:=\arg\inf_{\omega'}\lbrace \Upsilon_M(\omega')+3\Delta_C\|\omega'\|_2\rbrace
\end{align*}
satisfies
\begin{align*}
\wt\omega-\omega=-9\Delta_C^2\left(C^\top M C+9\Delta_C^2I\right)^{-1}\omega
\end{align*}
\end{lemma}
\begin{proof*}[ Lemma.~\ref{lemma:inf}]
First we consider the solution to the infimum optimization problem in the Eq.~\ref{eq:upperUpsilon}.
\begin{align*}
    \inf_{\omega'}\lbrace \Upsilon_M(\omega')+3\Delta_C\|\omega'\|_2\rbrace=\inf_{\omega'}\lbrace \|C\omega'-b\|_M+3\Delta_C\|\omega'\|_2\rbrace\leq \sqrt{2}\lbrace \sqrt{\inf_{\omega'}\lbrace\left(\|C\omega'-b\|_M\right)^2+\left(3\Delta_C\|\omega'\|_2\right)^2\rbrace}
\end{align*}
by taking the derivative of the the RHS and set it to zero:
\begin{align*}
    \nabla_{\omega'}\left(\|C{\omega'}-b\|_M+9\Delta_C^2\|\omega'\|_2^2\right)&=\nabla_{\omega'}\left(\left(C{\omega'}-b\right)^\top M \left(C\omega'-b\right)+9\Delta_C^2\|\omega'\|_2^2\right)\\
    &=\nabla_{\omega'}\left(\left(C\omega'\right)^\top M \left(C\omega'\right)-2\left(C\omega'\right)^\top M b+9\Delta_C^2\|\omega'\|_2^2\right)\\
    &=2A^\top M A\omega'-2C^\top M b +18\Delta_C^2\omega'\\
\end{align*}
by setting the last term equal to zero
\begin{align*}
0&=2C^\top M A\wt\omega-2C^\top M b +18\Delta_C^2\wt\omega\\
&\Longrightarrow C^\top M C\wt\omega +9\Delta_C^2\wt\omega=C^\top M b\\
&\Longrightarrow \left(C^\top M C+I\Delta_C\right)\wt\omega =C^\top M b\\
&\Longrightarrow \left(C^\top M C+9\Delta_C^2I\right)\wt\omega =C^\top M b\\
&\Longrightarrow \wt\omega =\left(C^\top M C+9\Delta_C^2I\right)^{-1}C^\top M b\\
\end{align*}
At the same time, for any $M$,  $\left(C^\top M C\right)\omega=C^\top M b$
as a result:
\begin{align*}
    \wt\omega &=\left(C^\top M C+9\Delta_C^2I\right)^{-1}C^\top M b=\left(C^\top M C+9\Delta_C^2I\right)^{-1}C^\top M C\omega\\
    &=\left(C^\top M C+9\Delta_C^2I\right)^{-1}\left(C^\top M C+9\Delta_C^2I\right)\omega^*-9\Delta_C^2\left(C^\top M C+9\Delta_C^2I\right)^{-1}\omega\\
    &=\omega-9\Delta_C^2\left(C^\top M C+9\Delta_C^2I\right)^{-1}\omega^*\\
    &\Longrightarrow \wt\omega-\omega=-9\Delta_C^2\left(C^\top M C+9\Delta_C^2I\right)^{-1}\omega
\end{align*}
for any vector $\varpi\in\Re^k$
\begin{align*}
\wt\omega-\omega=-9\Delta_C^2\left(C^\top M C+9\Delta_C^2I\right)^{-1}\omega
\end{align*}
\end{proof*}
\paragraph{Regularized estimator of $\omega^*$}
In low sample setting, when the number of observed samples from the target distribution is $m$ is low, the bound in theorem.~\ref{thm:concentration-theta} is vacuous. In this subsection we study the regularized version of \ose which sheds more light to the low sample size setting. In the theorem.~\ref{thm:concentration-theta}, we regularized the $\wh\omega$ around zero, while we might be more interested to regularized it toward vector of all ones, $\textbf{1}$, the importance wight such that there is not shift is considered. To analyze this setting, first we do the following change of variables;
\begin{align*}
    \omega:=\textbf{1}+\theta,\quad, \omega':=\textbf{1}+\theta',\quad \textit{and},\quad \wh\omega:= \textbf{1}+\wh\theta
\end{align*}
by this change of variables, we rewrite the measurement error problem as follows 
\begin{align}\label{eq:changeofvar}
    \Upsilon_M(\omega):=\|C\omega-b\|_M\Rightarrow \Upsilon_M(\omega):=\|C\left(\textbf{1}+\theta\right)-b\|_M\Rightarrow \Upsilon_M(\omega):=\|C\theta-\left(b-C\textbf{1}\right)\|_M
\end{align}
which results in the following change of variables  
\begin{align}\label{eq:changeofvar_hat}
 \wh\Upsilon_M(\omega):=\|\wh C\theta'-\left(\wh b-\wh C\textbf{1}\right)\|_M
\end{align}
under this change of variables, we can prove, the same way we did for \ref{thm:concentration-theta} the following Lemma.
\begin{lemma}\label{lemma:concentration-theta}
For the inverse problem in \ose with the change of variables in Eqs.~\ref{eq:changeofvar} and \ref{eq:changeofvar_hat} where $C$ and $\wh C$ are confusion matrix and its estimate, while $b=q_{h_0}$ and $\wh b=\wh q_{h_0}$, if the $\wh\theta$, as the solution to Eq.~\ref{eq:thetahat} is considered, for $\alpha=2$ and $M=I$, we have
\begin{align*}
\|\wh\theta-\theta\|_2\leq \frac{1}{\sigma_{min}}\left(\frac{2\|\theta\|_2\log\left(3k/\delta\right)}{(1-\beta)n}+\|\theta\|_2\sqrt{\frac{18\log\left(6k/\delta\right)}{(1-\beta)n}}+\sqrt{\frac{36\log\left(3/\delta\right)}{(1-\beta)n}}+\sqrt{\frac{36\log\left(3/\delta\right)}{m}}\right)
\end{align*}
with probablity at least $1-\delta$ for $\delta\leq 0.5$.
\end{lemma}
\begin{proof*}[ lemma.~\ref{lemma:concentration-theta}]
The proof if this lemma is straightforward after seeing the proof of theorem \ref{thm:concentration-theta}. The only change is instead of looking at $\|C-\wh C\|_2$ and $\|q_{h_0}-\wh q_{h_0}\|_2$ we need to look at $\|C-\wh C\|_2$ and $\|q_{h_0}-\wh q_{h_0}-C\textbf{1}+\wh C\textbf{1}\|$. The later part in short for the case of confusion matrix is $\|q_{h_0}-\wh q_{h_0}-p_{h_0}+\wh p_{h_0}\|$ and is upper bounded by 
\begin{align*}
\|q_{h_0}-\wh q_{h_0}-p_{h_0}+\wh p_{h_0}\|_2\leq\|q_h{0}-\wh q_{h_0}\|_2+\|p_{h_0}-\wh p_{h_0}\|_2 
\end{align*}
we have the concentration of $\|C-\wh C\|_2$ and $\|q_{h_0}-\wh q_{h_0}\|_2$ through lemmas.~\ref{lemma:C} and ~\ref{lemma:b}. Now, further we need the concentration over $\|p_{h_0}-\wh p_{h_0}\|_2$. The concentration over this term can be driven the same way as lemma.~\ref{lemma:b}. Therefore,
\begin{align*}
    \|\wh p_{h_0}-p_{h_0}\|\leq \frac{1}{\sqrt{(1-\beta)n}}+\sqrt{\frac{\log\left(1/\delta\right)}{(1-\beta)n}}
\end{align*}
As the results, with substituting this bounds into the analysis of the \ref{thm:concentration-theta} we have get the lemma statement.
\end{proof*}
This bound gives slightly different bound the $\omega$ version of it which does not have an addition term of $\sqrt{\frac{36\log\left(3/\delta\right)}{n}}$ but it depends on $\|\theta\|_2$ rather than $\|\textbf{1}+\theta\|_2$ which the first one can be significantly smaller the second one specially for the small shift setting. In the following we build our last step of regularization, we can build further regularization toward no-shift setting as follows in theorem.~\ref{thm:concentration-regularized}.
\begin{theorem}[Concentration of $\wh \theta$]\label{thm:concentration-regularized}
For the inverse problem in \ose with the change of variables in Eqs.~\ref{eq:changeofvar} and \ref{eq:changeofvar_hat} where $C$ and $\wh C$ are confusion matrix and its estimation, while same for $b=q_{h_0}$ and $\wh b=\wh q_{h_0}$ and same for $C\textbf{1}=p_{h_0}$ and $\wh C\textbf{1}=\wh p_{h_0}$, and the prior knowledge on upper bound of $\theta^*$ as $\|\theta\|_2\leq \theta_{\max}$, if the $\lambda$-shifted $\wh\theta$,~ $\wh\theta_\lambda:=\lambda\wh\theta$ is considered where $\wh\omega$ is the solution to Eq.~\ref{eq:thetahat} after the change of varibales , for $\alpha=2$ and $M=I$,
\begin{align*}
\|\wh\theta_\lambda-\theta\|_2\leq\min_{\lambda_\in\Lambda}\Bigg[ &\left(1-\lambda\right)\|\theta_{\max}\|_2+\frac{\lambda}{\sigma_{min}}\Bigg(\frac{2\|\theta_{\max}\|_2\log\left(3k|\Lambda|/\delta\right)}{(1-\beta)n}\\
&\quad\quad\quad~~+\|\theta_{\max}\|_2\sqrt{\frac{18\log\left(6k|\Lambda|/\delta\right)}{(1-\beta)n}}+\sqrt{\frac{36\log\left(3|\Lambda|/\delta\right)}{(1-\beta)n}}+\sqrt{\frac{36\log\left(3|\Lambda|/\delta\right)}{m}}\Bigg)\Bigg]
\end{align*}
with probability at least $1-\delta$ for $\delta\leq 0.5$.
\end{theorem}
\begin{proof*}
The proof is derivable by adding and subtracting trick and a further union bound on the set of $\lambda$. From lemma.~\ref{lemma:concentration-theta} and substituting $\|\theta_{\max}\|_2$ instead of $\|\theta^*\|_2$ on the RHS, we get
\begin{align*}
\|\wh\theta_\lambda-\theta\|_2&=\|\lambda\left(\wh\theta-\theta^*\right)-\left(1-\lambda\right)\theta^*\|_2\leq\|\lambda\left(\wh\theta-\theta^*\right)\|_2+\left(1-\lambda\right)\|\theta^*\|_2\\ &\leq\left(1-\lambda\right)\|\theta_{\max}\|_2+\frac{\lambda}{\sigma_{min}}\Bigg(\frac{2\|\theta_{\max}\|_2\log\left(3k/\delta\right)}{(1-\beta)n}\\
&\quad\quad\quad~~+\|\theta_{\max}\|_2\sqrt{\frac{18\log\left(6k/\delta\right)}{(1-\beta)n}}+\sqrt{\frac{36\log\left(3/\delta\right)}{(1-\beta)n}}+\sqrt{\frac{36\log\left(3/\delta\right)}{m}}\Bigg)
\end{align*}
since we know the value of each of the parts in the right hand side and since $\lambda\in\Lambda$ is a free variable, we can optimize over all possible $\lambda$'s in the set $\Lambda$. This optimization requires that the bound holds for all the lambdas, which means we need another union bound to get the theorem statement.
\end{proof*}
\begin{lemma}[Concentration of measurement matrix $\wh C$]\label{lemma:C}
Consider the definition of
\begin{align*}
    C=\E_{x,y\sim\D_p}\left[e_{h_0(x)}e_y^{\top}\right]
\end{align*}
where $e_i$ is one-hot-encoding of index $i$. Given the samples in data set $D_p$ and classifier $h_0$, we approximate $C$ through its empirical average of $\wh C=\frac{1}{(1-\beta)n}\sum_{(x_i,y_i)\in D_p}\left[e_{h_0(x_i)}e_{y_i}^{\top}\right]$
then 
\begin{align*}
    \|\wh C-C\|_2\leq \frac{2\log\left(2k/\delta\right)}{3(1-\beta)n}+\sqrt{\frac{2\log\left(2k/\delta\right)}{(1-\beta)n}}
\end{align*}
with probability at least $(1-\delta)$.
\end{lemma}
\begin{proof*} of Lemma\ref{lemma:C}.
We prove this lemma using the theorem 1.4[Matrix Bernstein] and Dilations technique from \citet{tropp2012user}. Consider a finite sequence $\lbrace\Psi_i\rbrace$ of independent random matrices with dimension $k$. By dilations, lets construct another sequence of self-adjoint random matrices of $\lbrace\wt\Psi_t\rbrace$ of dimension $2k$, such that $\forall{i}$ 
\[
   \wt\Psi_i=
  \left[ {\begin{array}{cc}
   \mathbf{0} & \Psi_i \\
   \Psi_i^\top & \mathbf{0} \\
  \end{array} } \right]
\] 
therefore,
\begin{align}\label{eq:dilationsuare}
   \wt\Psi_i^2=
  \left[ {\begin{array}{cc}
   \Psi_i\Psi_i^\top  & \mathbf{0} \\
   \mathbf{0} & \Psi_i^\top\Psi_i \\
  \end{array} } \right]
\end{align}
which results in $\|\wt\Psi_i\|_2=\|\Psi_i\|_2$. The dilation technique make translate the initial sequence of random matrices to the sequence of random self-adjoint matrices where we can apply Matrix Bernstein inequality. The Matrix Bernstein inequality theorem states that, for a finite sequence of i.i.d. self-adjoint matrices $\wt\Psi_i$, such that, almost surly  $\forall i, ~\E\left[\wt\Psi_i\right]=0$ and $\|\wt\Psi_i\|\leq R$, then for all $t\geq 0$, 
\begin{align*}
    \|\frac{1}{t}\sum_i^t\wt\Psi_i\|\leq \frac{R\log\left(2k/\delta\right)}{3t}+\sqrt{\frac{2\varrho ^2\log\left(2k/\delta\right)}{t}}
\end{align*}
with probability at least $1-\delta$ where $\varrho^2:=\|\E\left[\wt\Psi^2_i\right]\|_2,~\forall i$ which is also $\varrho^2=\|\E\left[\Psi^2_i\right]\|_2,~\forall i$ due to Eq.~\ref{eq:dilationsuare}. Therefore, thanks to dilation trick, \begin{align*}
    \|\frac{1}{t}\sum_i^t\Psi_i\|\leq \frac{R\log\left(2k/\delta\right)}{3t}+\sqrt{\frac{2\varrho ^2\log\left(2k/\delta\right)}{t}}
\end{align*}
with probability at least $1-\delta$. 

Now, by plugging in $\Psi_i=e_{h_0(x_i)}e_{y_i}^{\top}-C$, we $\E\left[\wt\Psi_i\right]=0$. We also have $\|\wt\Psi_i\|\leq 2$ as well as $\varrho^2=\|\E\left[\Psi^2_i\right]\|_2=1$. therefore, if $t=N$ we have
\begin{align*}
    \|\wh C-C\|_2\leq \frac{2\log\left(2k/\delta\right)}{3(1-\beta)n}+\sqrt{\frac{2\log\left(2k/\delta\right)}{(1-\beta)n}}
\end{align*}
\end{proof*}



\begin{lemma}\label{lemma:b}[Concentration of measurements] Consider the set of $m$ sampels of target set $D_q$. After applying hypothesis $h_0$ on $x$'s in $D_q$, we generate a set with elements $\lbrace h_0(x_i)\rbrace_i^m$. Further, consider the definition of $q_{h_0}=\E_{x\sim \D_q(\X)}\left[e_{h_0(x)}\right]$. Given the sample set of $\lbrace h_0(x_i)\rbrace_i^m$ and empirical estimate of the $q_{h_0}$ as $\wh q_{h_0}=\frac{1}{m}\sum_i^me_{h_0(x_i)}$, then
\begin{align*}
    \|\wh q_{h_0}-q_{h_0}\|\leq \frac{1}{\sqrt{m}}+\sqrt{\frac{\log\left(1/\delta\right)}{m}}
\end{align*}
with probability at least $1-\delta$.

\end{lemma}
\begin{proof*} of Lemma.~\ref{lemma:b}. The proof of this lemma is mainly based on a special case of and appreared at proposition 6 in \citet{azizzadenesheli2016reinforcement}, Lemma F.1 in \citet{anandkumar2012method} and Proposition 19 of \citet{hsu2012spectral}. Consider a fixed multinomial distribution characterized with probability vector of $\wb\varsigma\in\Delta_{k-1}$ where $\Delta_{k-1}$ is a $k-1$ dimensional simplex. Further, consider $t$ realization of this multinomial distribution $\lbrace\varsigma_i\rbrace_{i=1}^t$ where $\varsigma_i$ is the one-hot-encoding of the $i$'th sample. Consider the empirical estimate mean of this distribution through empirical average of the samples; $\wh\varsigma=\frac{1}{t}\sum_i^t\varsigma_i$, then 
\begin{align*}
    \|\wh\varsigma-\wb\varsigma\|\leq \frac{1}{\sqrt{t}}+\sqrt{\frac{\log\left(1/\delta\right)}{t}}
\end{align*}
with probability at least $1-\delta$.

By plugging in $\wb\varsigma=q_{h_0}$, $\wh\varsigma=\wh q_{h_0}$, and $t=m$ and finally $\lbrace\varsigma_i\rbrace_{i=1}^m=\lbrace e_{h_0(x_i)}\rbrace_i^m$ we get the statement in Lemma.~\ref{lemma:b}
\end{proof*}

==> Old/Generalization.tex <==
\section{Generalization bound}







In this section, we investigate the generalization characteristics of \ose. In order to make the analysis of the generalization concert, we provide the following characteristics of the importance weights.
\begin{align}\label{eq:iw-property}
    \E_p[w_Y] = 1,\quad \E_p[w_Y^2] = d(q||p), \quad \sigma^2_p(w_Y)=d(q||p)-1
\end{align}
The $\E_p[w_Y] = 1$ is valid since $\E_p[w_Y] = \sum_i^kp_i\frac{q_i}{p_i}$. As followed, $\E_p[w_Y^2]=\sum_i^kp_i\frac{q^2_i}{p^2_i}=\sum_i^kq_i\frac{q_i}{p_i}$ and then finally the variance equality follows. 

Furthermore the second moment of the importance weighted loss $\E_{D_p}\left[\omega_Y^2l^2(Y,h(X))\right]$, given a $h\in\HH$, is also bounded. For an $\alpha\geq 0$;

\begin{align}
    \E_{\D_p}\big[&\omega_Y^2l^2(Y,h(X))\big]\nonumber\\
    &=\sum_i^k p_i \frac{q^2_i}{p^2_i}\E_{X\sim \D_p|Y=i}\left[l^2(i,h(X))\right]\nonumber\\
    &=\sum_i^k q_i^{\frac{1}{\alpha}} \frac{q_i}{p_i}q_i^{\frac{\alpha-1}{\alpha}}\E_{X\sim \D_p|Y=i}\left[l^2(i,h(X))\right]\nonumber\\
    &\leq\left(\sum_i^k q_i \frac{q_i^\alpha}{p_i^\alpha}\right)^{\frac{1}{\alpha}}\left(\sum_i^kq_i\E_{X\sim \D_p|Y=i}\left[l^2(i,h(X))\right]^{\frac{2\alpha}{\alpha-1}}\right)^{\frac{\alpha-1}{\alpha}}\nonumber\\
    &=\left(\sum_i^k q_i \frac{q_i^\alpha}{p_i^\alpha}\right)^{\frac{1}{\alpha}}\left(\sum_i^kq_i\E_{X\sim \D_p|Y=i}\left[l^2(i,h(X))\right]\E_{X\sim \D_p|Y=i}\left[l^2(i,h(X))\right]^{\frac{\alpha+1}{\alpha-1}}\right)^{\frac{\alpha-1}{\alpha}}\nonumber\\
    &\leq\left(\sum_i^k q_i \frac{q_i^\alpha}{p_i^\alpha}\right)^{\frac{1}{\alpha}}\sum_i^kq_i\E_{X\sim \D_p|Y=i}\left[l^2(i,h(X))\right]^{1-\frac{1}{\alpha}}\E_{X\sim \D_p|Y=i}\left[l^2(i,h(X))\right]^{1+\frac{1}{\alpha}}
\end{align}
Where the first inequality follows from Holder's inequality and the second one follows from Jensen's inequality and the fact that the loss is in $[0,1]$ and the function is convex in this region. Moreover, since $1+\frac{1}{\alpha}\geq 1$ and upper bound for the loss square, $l(\cdot,\cdot)^2\leq 1$, then;
\begin{align*}
    \E_{\D_p}\big[&\omega_Y^2l^2(Y,h(X))\big]\leq\left(\sum_i^k q_i \frac{q_i^\alpha}{p_i^\alpha}\right)^{\frac{1}{\alpha}}\sum_i^kq_i\E_{X\sim \D_p|Y=i}\left[l^2(i,h(X))\right]^{1-\frac{1}{\alpha}}
\end{align*}
which gives bound on the second moment of weighted loss. If one prefers a specific $\alpha$ or has prior knowledge that RHS is small enough for a given $\alpha$ then the bound for that $\alpha$ of interest can be used. In our study, we set $\alpha=1$ and get
\begin{align}\label{eq:second-moment}
    \E_{\D_p}\big[\omega_Y^2l^2(Y,h(X))\big]\leq d(q||p)
\end{align}
which is also simply could be driven by $\E_{\D_p}\big[\omega_Y^2l^2(Y,h(X))\leq \E_{\D_p}\big[\omega_Y^2)$ then applying applying second characteristics in Eq.~\ref{iw-property}.
Since we have a bound on the second moment of weighted loss while its first moment is $L(h)$ we can apply Bernstein's inequality 
\begin{lemma}[Concentration of weighted loss]\label{lemma:single-h} For a give hypothesis $h\in\HH$, $n$ sample from the source data set, and access to the importance weights $\omega$ we have;
\begin{align*}
    |\wh L(h)-L(h)|\leq \frac{d_\infty(q||p)\log(\frac{2}{\delta})}{3\beta n}+\sqrt{\frac{2\left(d(q||p)-L(h)^2\right)\log(\frac{2}{\delta})}{\beta n}}
\end{align*}
with probability at least $1-\delta$
\end{lemma}
\begin{proof*} of Lemma.~\ref{lemma:single-h}.
Let's $d_\infty(q||p):=\sup_i\frac{q_i}{p_i}$
Consider a random variable $\omega_Yl(Y,h(X)$. Through target set, we have a data set $D_p$ of $n$ samples. Therefore, since $L(h)$ which is an expectation of $\wh L(h)$, due to Bernstein's inequality for a zero mean random variable $\wh L(h)-L(h)$ with upper bound on variance  $d(q||p)-L(h)^2$, we have the statement of the theorem.~\ref{lemma:single-h}
with probability at least $1-\delta$
\end{proof*}
The theorem.~\ref{lemma:single-h} give the concentration result of a fixed hypothesis, while for generalization, we have the union bound step left. 
\begin{theorem}[Union bound over the finite hypothesis class $\HH$]\label{thm:finite-h} Given a finite hypothesis class $\HH$ with cardinally of $|\HH|$, $n$ sample from the source data set, and access to the importance weights $\omega$, a simple application of union bound results in 
\begin{align*}
    \sup_{h\in\HH}|\wh L(h)-L(h)|\leq \frac{d_\infty(q||p)\left(\log(|\HH|)+\log(\frac{2}{\delta})\right)}{3\beta n}+\sqrt{\frac{2\left(d(q||p)\right)\left(\log(|\HH|)+\log(\frac{2}{\delta})\right)}{\beta n}}
\end{align*}
with probability at least $1-\delta$. This directly states that
\begin{align*}
    |L(\wh h)-L(h^*)|\leq \frac{2d_\infty(q||p)\left(\log(|\HH|)+\log(\frac{2}{\delta})\right)}{3\beta n}+\sqrt{\frac{8\left(d(q||p)\right)\left(\log(|\HH|)+\log(\frac{2}{\delta})\right)}{\beta n}}
\end{align*}
with probability at least $1-\delta$
\end{theorem}
The stated generalization bound in the Theorem\ref{thm:finite-h} assume the access to the importance weights while we also need to estimate it. Let, for given hypothesis $h\in\HH$, $\wh L(h;\wh\omega)$ denote the loss under approximated importance weight $\wh\omega$;
\begin{align*}
    \wh L(h;\wh\omega)=\frac{1}{\beta n}\sum_{(x_i,y_i)\in D_p^\beta }\wh\omega_{y_i}l(y_i,h(X_i))
\end{align*}
By addition and subtraction we have
\begin{align}\label{eq:decom}
    |\wh L(h;\wh\omega)-L(h)|&=|\wh L(h;\wh\omega)-\wh L(h)+\wh L(h)-L(h)|\leq\underbrace{|\wh L(h;\wh\omega)-\wh L(h)|}_\text{(a)}+\underbrace{|\wh L(h)-L(h)|}_\text{(b)} \nonumber\\
\end{align}
The term $(a)$ represent deviating due to the estimation error in importance weight and the second term $(b)$ represents the concentration to the expected loss. The second term $(b)$ is bounded in Lemma.~\ref{lemma:single-h}. 

\begin{align*}
    (a):|\wh L(h;\wh\omega)-\wh L(h)|=\frac{1}{\beta n}|\sum_{(x_i,y_i)\in D_p }\left(\wh\omega_{y_i}-\omega_{y_i}\right)l(y_i,h(X_i))|
\end{align*}
consider a transformation $\phi:\Y\times \Re\rightarrow \Re^k$ which take pair of $(y,l(y,h(X)))$ and turn it to a $k$ dimensional vector of all zeros, except $l(y,h(X))$ in $y$'th entry. Therefore,
\begin{align*}
    (a):|\wh L(h;\wh\omega)-\wh L(h)|&=\frac{1}{\beta n}|\sum_{(x_i,y_i)\in D_p }\left(\wh\omega-\omega\right)^\top \phi(y_i,l(y_i,h(X_i)))|\nonumber\\
    &\leq\frac{1}{\beta n}\|\wh\omega-\omega\|_2 \|\Phi_{D_p}\|_2\nonumber\\ 
\end{align*} 
where $\Phi_{D_p}\in\Re^{k\times n}$ and its $i$'th column is equal to $\phi(y_i,l(y_i,h(X_i)))$. Since $\|\Phi_{D_p}\in\Re^{k\times n}\|_2\leq n$ then,
\begin{align*}
    (a):|\wh L(h;\wh\omega)-\wh L(h)|\leq\|\wh\omega-\omega\|_2 
\end{align*} 
while through theorem \ref{eq:thetahat}, we have
\begin{align*}
    (a):|\wh L(h;\wh\omega)-\wh L(h)|\leq \frac{1}{\sigma_{min}}\left(\frac{2\|\omega\|_2}{(1-\beta)n}+\|\omega\|_2\sqrt{\frac{18\log\left(4k/\delta\right)}{(1-\beta)n}}+\sqrt{\frac{36\log\left(2/\delta\right)}{m}}\right)
\end{align*} 
Consider $\wh h_{\wh\omega}:=\arg\min_{h\in\HH}\wh L(h;\wh\omega)$. Combining $(a)$, $(b)$ and the union bound we have the following theorem.
\begin{theorem}[Generalization Bound of finite hypothesis class $\HH$]\label{thm:gen}
Given a finite hypothesis class $\HH$ with cardinally of $|\HH|$, $n$ sample from the source data set, $m$ sample input from target set results in the following generalization bound.
\begin{align*}
    |L(\wh h_{\wh\omega})-L(h^*)|&\leq \frac{2d_\infty(q||p)\left(\log(|\HH|)+\log(\frac{3}{\delta})\right)}{3\beta n}+\sqrt{\frac{8\left(d(q||p)\right)\left(\log(|\HH|)+\log(\frac{3}{\delta})\right)}{\beta n}}\nonumber\\
    &\quad\quad+\frac{2}{\sigma_{min}}\left(\frac{2\|\omega\|_2}{(1-\beta)n}+\|\omega\|_2\sqrt{\frac{18\log\left(6k/\delta\right)}{(1-\beta)n}}+\sqrt{\frac{36\log\left(3/\delta\right)}{m}}\right)
\end{align*}
with probability at least $1-\delta$
\end{theorem}



\begin{lemma}[Generalization Bound of finite hypothesis class $\HH$with reparameterization trick]\label{thm:gen-reparam}
Given a finite hypothesis class $\HH$ with cardinally of $|\HH|$, $n$ sample from the source data set, $\beta$ as the splitting factor, $m$ sample input from target set, with $\wh\omega=\textbf{1}+\wh\theta$, as $\wh\theta$ the output of reparameterized \ose, we have
\begin{align*}
    |L(\wh h_{\wh\omega})-L(h^*)|&\leq \frac{2d_\infty(q||p)\left(\log(|\HH|)+\log(\frac{3}{\delta})\right)}{3\beta n}+\sqrt{\frac{8\left(d(q||p)\right)\left(\log(|\HH|)+\log(\frac{3}{\delta})\right)}{\beta n}}\nonumber\\
    &\left(1-\lambda\right)\|\theta\|_2+\frac{\lambda}{\sigma_{min}}\Bigg(\frac{2\|\theta\|_2\log\left(3k/\delta\right)}{(1-\beta)n}\\
&\quad\quad\quad~~+\|\theta_{\max}\|_2\sqrt{\frac{18\log\left(6k/\delta\right)}{(1-\beta)n}}+\sqrt{\frac{36\log\left(3/\delta\right)}{(1-\beta)n}}+\sqrt{\frac{36\log\left(3/\delta\right)}{m}}\Bigg)
\end{align*}
with probability at least $1-\delta$
\end{lemma}

\begin{theorem}[Generalization Bound with optimal data ration and regularization]\label{thm:gen-reparam-opt}
Given a finite hypothesis class $\HH$ with cardinally of $|\HH|$, $n$ sample from the source data set, splitting set $\B$, regularization set $\Lambda$, $m$ sample input from target set, with $\wh\omega=\textbf{1}+\wh\theta$, as $\wh\theta$ the output of reparameterized \ose, we have
\begin{align*}
    |L(\wh h_{\wh\omega})-L(h^*)|&\leq\min_{\beta\in\B}\Bigg\{ \frac{2d_\infty\left(\log(|\HH|)+\log(\frac{3|\B|}{\delta})\right)}{3\beta n}+\sqrt{\frac{8\left(d_{\max}\right)\left(\log(|\HH|)+\log(\frac{|\B|3}{\delta})\right)}{\beta n}}\nonumber\\
    &\min_{\lambda_\in\Lambda}\Bigg\{\left(1-\lambda\right)\|\theta_{\max}\|_2+\frac{\lambda}{\sigma_{min}}\Bigg(\frac{2\|\theta_{\max}\|_2\log\left(3k|\B||\Lambda|/\delta\right)}{(1-\beta)n}\\
&~~+\|\theta_{\max}\|_2\sqrt{\frac{18\log\left(6k|\B||\Lambda|/\delta\right)}{(1-\beta)n}}+\sqrt{\frac{36\log\left(3|\B||\Lambda|/\delta\right)}{(1-\beta)n}}+\sqrt{\frac{36\log\left(3|\B||\Lambda|/\delta\right)}{m}}\Bigg)\Bigg\}\Bigg\}
\end{align*}
with probability at least $1-\delta$ where $d_\infty$ is prior knowledge on maximum possible $d_\infty(q||p)$ and $d_{\max}$ the prior knowledge on maximum possible $d(q||p)$.
\end{theorem}

\begin{theorem}[Generalization Bound for online setting]\label{thm:gen-reparam-opt-online}
Given a finite hypothesis class $\HH$ with cardinally of $|\HH|$, $n$ sample from the source data set, splitting set $\B$, regularization set $\Lambda$, $m$ sample input from target set, with $\wh\omega=\textbf{1}+\wh\theta$, as $\wh\theta$ the output of reparameterized \ose, at each time step $t$ with $t$ observation from the target domain, we have $\forall i\leq t, i\in \N$
% \begin{align*}
%     |L(\wh h_{\wh\omega^t}^t)&-L(h^*)|\leq\min_{\beta\in\B}\Bigg\{ \frac{2d_\infty\left(\log(|\HH|)+\log(\frac{3T|\B|}{\delta})\right)}{3\beta n}+\sqrt{\frac{8\left(d_{\max}\right)\left(\log(|\HH|)+\log(\frac{T|\B|3}{\delta})\right)}{\beta n}}\nonumber\\
%     &\min_{\lambda_\in\Lambda}\Bigg\{\left(1-\lambda\right)\|\theta_{\max}\|_2+\frac{\lambda}{\sigma_{min}}\Bigg(\frac{2\|\theta_{\max}\|_2\log\left(3kT|\B||\Lambda|/\delta\right)}{(1-\beta)n}\\
% &~~+\|\theta_{\max}\|_2\sqrt{\frac{18\log\left(6kT|\B||\Lambda|/\delta\right)}{(1-\beta)n}}+\sqrt{\frac{36\log\left(3T|\B||\Lambda|/\delta\right)}{(1-\beta)n}}+\sqrt{\frac{36\log\left(3T|\B||\Lambda|/\delta\right)}{m}}\Bigg)\Bigg\}\Bigg\}
% \end{align*}
\begin{align*}
    |L(\wh h_{\wh\omega^i}^i)&-L(h^*)|\leq\min_{\beta\in\B}\Bigg\{ \frac{2d_\infty\left(\log(|\HH|)+\log(\frac{3T|\B|}{\delta})\right)}{3\beta n}+\sqrt{\frac{8\left(d_{\max}\right)\left(\log(|\HH|)+\log(\frac{t|\B|3}{\delta})\right)}{\beta n}}\nonumber\\
    \!\!\!\!\!\!\!&\min_{\lambda_\in\Lambda}\Bigg\{\left(1-\lambda\right)\|\theta_{\max}\|_2+\frac{\lambda}{\sigma_{min}}\Bigg(\frac{2\|\theta_{\max}\|_2\log\left(3kt|\B||\Lambda|/\delta\right)}{(1-\beta)n}\nonumber\\
&~~\!\!\!\!\!\!\!+\|\theta_{\max}\|_2\sqrt{\frac{18\log\left(6kt|\B||\Lambda|/\delta\right)}{(1-\beta)n}}+\sqrt{\frac{36\log\left(3t|\B||\Lambda|/\delta\right)}{(1-\beta)n}}+\sqrt{\frac{36\log\left(3t|\B||\Lambda|/\delta\right)}{m}}\Bigg)\Bigg\}\Bigg\}
\end{align*}
with probability at least $1-\delta$ where $d_\infty$ is prior knowledge on maximum possible $d_\infty(q||p)$ and $d_{\max}$ the prior knowledge on maximum possible $d(q||p)$.
\end{theorem}


The theoretical analysis of this section is mainly inspired by literature and materials in generalization theory specially, Percy Liang course not at Statistics 231/CS229T: Statistical Learning Theory, as well as Peter Bartlett's and Sasha Rakhlin's course, more specifically, \citep{ben2007analysis,cortes2010learning}.

\paragraph{Bound with no knowledge of the shift parameters}

==> Old/old-3-Preliminaries.tex <==
\section{Preliminaries}
We denote $\X$ as the space of input and $\Y$ as categorical space of labels $\Y=\left[k\right]=\lbrace 1,\ldots,k\rbrace$ as a set of classes/categories.  We express the joint distribution input-label $(x,y)\in \X\times\Y$ in source domain $\S$ as $\D_p$ and in target domain $\T$ as $\D_q$. Correspondingly, we denote $p$ and $q$ as the marginal probability mass functions over labels in the source and the target domain, while the data set of samples from source is denoted as $D_p$ and for target as $D_q$. It worth noting that $D_q$ does not contain labels of target set. The cardinally of source data set is depicted as $n$ and for target as $m$ unless specified otherwise. Moreover, we use $\D_p(\X)$ as the marginal distribution of inputs in source as well as $\D_q(\X)$ for target. 

\paragraph{Problem set-up}
Let $h_0$ denote as a given memory less hypothesis for the classification task (might be useful classifier) which we do not have access to unless through query calls of inputs. Let $p_{h_0}$ denote the label distribution when we apply $h_0$ to source data and $q_{h_0}$ the counter part of target domain. Moreover, let $\wh p_{h_0},\wh q_{h_0}\in\Re_+^k$ denote their empirical approximation. 
For the label shift problem of interest, the anti-causal setting; we have
\begin{align}\label{eq:anti-causal}
    \D_p(\cdot|y)=\D_q(\cdot|y),~\forall y\in\Y
\end{align}
Furthermore, we require $\forall y\in \Y$, if $q(y)\geq 0$, then $p(y)\geq 0$. This is a reasonable setting since without any further prior knowledge, there is no way to properly reason about a class that does not exist in the source domain but appears in the target. Moreover, we need $h_0$ to be useful in some sense. For example if $h_0$ almost always output a fix class, then it does not capture any characteristics of the the data. Therefore, we are interested in the classifier which does not results in singularity in the spectrum of confusion matrix, i.e.
\begin{align*}
    C=\D_p(Y',Y)
\end{align*}
is full rank matrix where $Y':=h_0(X)$. If this matrix is singular, therefore class distributing is not identifiable under $h_0$. For example if two rows of $C$ are same, therefore there are two classes, $i$ and $j$ that $h_0$ assigns any true label identically to either $i$ or $j$ with the same probability which is a pathological setting. We define $\omega$ as the importance weight between these two domain $\omega_i=\frac{q(y=i)}{p(y=i)}=\frac{q_i}{p_i}$ and a notion of shift as $d(\D_q||\D_p)=d(q||p)=:\E_q\left[\omega_YY\right]=\sum_i^kq_i\frac{q_i}{p_i}$. We just look at class distribution since due to anti-causal setting, 
\begin{align*}
\frac{\D_q(X,y=i)}{\D_p(X,y=i)}=\frac{\D_q(X|y=i)q_i}{\D_p(X|y=i)p_i}=\frac{q(y=i)}{p(y=i)}
\end{align*}
We measure the shift by $d(\D_q||\D_p)$, which is equivalent to the exponent of second order Renyi divergence. Given a hypothesis class $\HH$, a loss function $l:\Y\times\Y\rightarrow [0,1]$ we define the expected loss of a classifier $h\in\HH$ as 
\begin{align*}
    L(h)=\E_{X,Y\sim\D_p}\left[\omega_Yl(Y,h(X))\right]=\E_{X,Y\sim\D_q}\left[l(Y,h(X))\right]
\end{align*}
Therefore, in order to find the classifier which generalize well in target set, we minimize the empirical weighed risk. 


==> Old_1-Introduction_0925.tex <==
\section{Introduction}

In the supervised learning paradigm, the task to make predictions on a given but unlabeled \emph{target} set is usually solved by training a predictive model on a labeled \emph{source} set. This is a sensible approach in particular when the source and target samples are expected to be samples from the same distribution. However, this assumption does not hold in many
real-world applications. 

%We want to demonstrate the problem of \emph{distributional shift} in two scenarios related to medical applications, while it arises in many other domains as well.

For example, oftentimes predictions for medical diagnostics are based on data from a particular population of patients and machines due to the limited variety of data that is available in the
training phase. In particular, our framework addresses the following scenario:
A classifier is trained to predict whether a patient has attracted(?) a severe disease in country A based on physical measurements and diagnosis (labeled source data). The disease is potentially even more prevalent in country B, where however only few experts are available to make a diagnosis. Most importantly, the diagnosis is currently made by the doctors using an unknown combination of symptom descriptions, measurements and other soft signals they can pick out. The following questions might be relevant for the data scientists
\begin{itemize}[leftmargin=1.5em ]
    \item If we send a group of volunteers to country B with the same equipment to 
    record measurements of patients, how can the data in country A and the new unlabeled data from country B be used to
    update the classifier to give good diagnostic predictions for patients in country B?
    %\item If our classifier diagnose a set of disease given a set of symptom in country A, can it also do well in a new country B?
    %\item  can we use this data and update the model to diagnose disease better?%they just locally update
    \item If the patients in country B come in slowly over time and the disease is deadly, can the
    classifier be updated after each patient is measured, so as to maximize the
    accuracy of the performance for the next patient? 
    %If the diseases are dangerous and are needed to be diagnose quickly, can this group locally update the model online, patient after patient?
    Similarly, the disease might spread very fast in country A after an unexpected event. Can we detect and adapt to the new disease distribution quickly when measuring the measurements one patient at a time? 
    %\fycomment{this could be merged with above point?}\Kamyar{Mathematically they are talking about the same thing}
\end{itemize}
Similar problems arise in many other domains besides health-care, such as recognition and reconstruction tasks, where the input represent the underlying object. We will use this medical example throughout the paper for ease of presentation.
%\anima{i would not state it this way. it seems to apply u are solving this specific healthcare problem. may be phrase it as: consider the following scenario. and then after u report the bullet points, say there are indeed many other settings where such problems arise.}

\fycomment{are we also discussing what is "good" (f-1 /accuracy etc. at some point?)}
% We develop importance wi
% a method with generalization guarantee that helps us to do better in such situations. Our model is able to handle exponentially and combinatorially many configuration of disease per human while not losing and degrading its performance.
%\section{Domain adaptation for distributional shifts}
%% In this section we briefly illuminate the setting in which our contribution is based on, while introducing some notation that is used throughout the paper.
% \Kamyar{health care motivation can be helpful why this problem is a significant one to tackle.}


% In a typical prediction task, data scientists are faced with the problem of developing a model which can make good predictions on data $x,y\in\X\times\Y$ in a \emph{target} set, which are sampled from a joint distribution $\disQ$. However, the labels on the target set $y$'s are not known. Instead they use a \emph{source} data set with samples from the distribution $\disP$. In usual supervised learning tasks in machine learning, it is assumed $\disQ = \disP$  so that there is hope of generalization. However when this assumption does not hold in many applications and we still desire to obtain good predictive performance and generalization, it is generally called domain adaptation.\anima{no where here have u mentioned that samples are drawn iid. and u haven't explicitly spelled out what is x and y}\fycomment{i.i.d. is not the key here, could also be HMMs? important here is that we have samples from distribution?}
 
% \subsection{Covariate shift}
If we view the data, consisting of an input $x \in \X$ and a label $y$ in a finite domain $\Y$, in the source and target set as samples from joint distributions $\disP$ and $\disQ$, we are statistically dealing
with the fact that $\disP \neq \disQ$, also known as distributional shift.
%Problems where the source distribution $\disP$ is not equivalent to the target distribution $\disQ$
%belong to the general field of domain adaptation and distributional shift. 
The difference between $\disP$ and $\disQ$ can be modeled in many different ways based on the use case at hand.~\citet{scholkopf2012causal} studies two main perspectives: (i) causal learning assumes that the explanatory input $x$ causes the label $y$ whereas in the $(ii)$ anti-causal setting, the label $y$ causes the input $x$. 

For the causal setting, one usually assumes that the marginal distribution of the covariates $x$ shifts from $\disP$ to $\disQ$, where as the conditional probability of $y$ given $x$ stays constant.
This assumption is sensible when there is reason to believe that there is a true optimal mapping from $x$ to $y$ which
does not change if the distribution of $x$ changes.  As an example,
if a given set of symptoms correctly predicts a disease for the
``right reasons'', the predictive function should be the same, no
matter which country you are moving to. Various methods have been developed in the extensive literature targeting the \emph{covariate shift} setting
%has been studied extensively in the literature, 
see e.g. importance weighting (reference), KMM, xyz~\citep{shimodaira2000improving}.

% Although it is correct that
% an optimal and robust mapping should stay constant throughout
% different domains, in most cases this assumption is not satisfied by
% the actual distributions $\disP$ and $\disQ$.
%The former is built on the  of covariate shift and the latter is on label shift. In covariate shift, the observed covariate follows a different distribution as in target $\disQ$ and the source $\disP$. 
% In covariate shift literature, the data is described as pairs of explanatory, i.e. input $x$, and the response, $y$, i.e. the label~\citep{shimodaira2000improving} where the assumption is that $y$ is the response to $x$, i.e. the causal setting. 
%\anima{please use   ~ (sim symbol) next to citation. }
%In the label shift, the label \anima{$y$} follows different distributions as in target $\disQ$ and the source $\disP$ while the label $y$ derives the distribution over the observation $x$. 
Although many of these methods
have theoretical guarantees, their dependence in the input dimension has made it 
difficult to apply them to large datasets. Furthermore, going back to our motivating example, we can see that the causal setting alone does not capture the nature of many other practical use cases - that is, the covariate shift assumption is not satisfied.

Specifically, in a lot of data science applications there is an inherent truth $y$ that 
we want to learn given observations $x$, which can be "explained" by $y$. 
For example, the physical symptoms reported by a patient might be approximately similar among all sick patients. This simplified
relation can be modeled by the structural equation model (SEM) $x = f(y, \nu)$ where $\nu$ is independent noise or a directed graphical model $Y \to X$. However, the percentage of ill patients in the two countries A and B may be very different, i.e. $\disP(Y = i) \neq \disQ(Y=i)$. 
Similarly, within one country, the number of ill patients may suddenly change because of an irregular event such as a natural catastrophe. 

\begin{wrapfigure}{t}{.45\textwidth}
% \begin{minipage}{1.\textwidth}
  \centering
  \footnotesize
  \begin{tabular}{c|c}
    \multicolumn{1}{c}{Covariate Shift }&\multicolumn{1}{c}{Label Shift} \\
    \toprule
 \makecell{$\disP(X)\neq\disQ(X)$\\$\disP(Y|X)=\disQ(Y|X)$}  & \makecell{$\disP(Y)\neq\disQ(Y)$\\$\disP(X|Y)=\disQ(X|Y)$}\\
    \bottomrule
  \end{tabular}
  \vspace*{-.5cm}
%   \label{table:settings}
% \end{minipage}
\end{wrapfigure}

In all of the above cases, the shift is in the distribution of the label $y$ (sick or healthy), while given a fixed label, the conditional distribution of $x$ given $y$ is constant.
By the Bayes rule, the \emph{label shift} causes the covariate shift condition
to be violated, i.e.  $\disP(Y|X = x) \neq \disQ(Y|X=x)$. Despite
being a natural scenario, even this simplified model has not yet been
sufficiently studied in the literature.
In contrast to covariate shift,
reweighting the samples in the source set is not straight-forward
since the marginal distribution of $Y$ in distribution $\disQ$
cannot be directly estimated.
%which is a gap we aim to fill with this work. 

% Let us first consider the toy case where the symptoms $x$ can be
% mainly ``explained'' by the label $y$. This is how data science
% usually works: there is an underlying and inherent truth of the data
% that we observe, which depends on $y$ that we really want to
% learn. For example, a disease causes symptoms, a person causes a
% picture and so on. If we simplistically \anima{simplistically is not typically used. naively?} assume that indeed $x =
% f(y,\nu)$ where $\nu$ is some noise, 
% then any shift in the labels, that is
% $\disP(Y = i) \neq \disQ(Y=i)$, causes the covariate shift condition
% to be violated, i.e.  $\disP(Y|X = x) \neq \disQ(Y|X=x)$ by the Bayes
% rule, whereas the label shift assumption holds by definition. Despite
% being a natural scenario, even this simplified model has not yet been
% sufficiently studied in the literature which is a gap we aim to fill
% with this work. 

% Consider in our two countries, the distribution of diseases is different, while the driven distribution of symptoms by disease stays same. For example the distribution of pneumonia might be different in two countries, but fairly similar symptoms behaviour is exported from two patients diagnosed to have pneumonia but one from the country A and other from B. Furthermore, consider in the country A, after an event, the pneumonia distribution changes among the people and we are interested in adapting to this change by data we collect every day, even after each patient is visited. A similar motivation, for \anima{for is not correct.. in} batch setting is provided in~\cite{lipton2018detecting}. \anima{batch suddenly jumped out. in previous paragraph u should mention both streaming and batch} \anima{also too early to introduce Zack's paper. i will mention place to introduce later}

% \subsection{A case for label shift}
% Motivated by the health care and disease diagnosing problems \anima{u can just say disease diagnosis}, as well as many other applications, such as Recognition and Reconstruction tasks \anima{no need for capitalization}, where the input represent the underlying object \anima{i have no idea what this means}, \fycomment{moved this above}

% One may object that even the label shift assumption could be overly simplified for some real world situations, in particular the symptoms could also depend on unobserved confounders. Albeit being valid concerns, our setting is evidently a basic and important one which needs to be solved first, before more complicated 
% and realistic ones may follow. Due to the fact that surprisingly few papers have tackled the \emph{label shift} setting before, this paper aims at proposing a new method as well as generalization guarantees for an estimator which has access to the entire labeled source data and full or streaming access to unlabeled target data.  

% More formally, in the following sections we consider classification tasks where the random variables $X,Y$ take values $x\in \R^d$ and $y\in\Y:= \left[k\right]=\lbrace 1,\ldots,k\rbrace$. We study the case that conditional distributions are equivalent in both domains, i.e. $\disP(X=x|Y=i) = \disQ(X=x|Y=i)$ for all $x\in \X$ and $y \in [k]$. The marginal distributions on $Y$ however can differ. \fycomment{not quite sure whether it's good to do general domains $\X, \Y$ first before going to the discrete $Y$ domain which makes conditional dist. notation much cleaner while math. correct}


% Generally, many real-world applications can be framed in label shift graphical model \ with invariant conditional
% $X|Y$ instead of $Y|X$.  

%For example, if a disease $y$ can be uniquely identified from symptoms $x$ including some irrelevant features, it is natural that if the labels correlate with invariant features in the t
% \fycomment{probably need to move to the covariate shift passage}

% On the contrary the following kind of shift appears regularly during
% data collection: when the percentage of labels of each class differ
% more or less in the source and target set. In the previous binary example,
% this would correspond to a different percentage of sick patients for different diseases
% in different countries.



\noindent{\bf Contributions: } This paper aims to fill the gap in terms of both theoretical understanding
and practical methods for the label shift setting and thereby move a step closer towards more complicated and realistic
distributional shift models. 
\citet{lipton2018detecting} have introduced a provably good importance weight estimator which has access to the entire labeled source data set and the entire batch of unlabeled target data (which we call the \emph{batch} setting), and demonstrated promising performance on real data. There are a two natural follow-up questions which remain unanswered by their work: What are the generalization guarantees for the final predictor which uses the importance weighted samples? How do we deal with the uncertainty of the importance weights estimation in the \emph{streaming} setting, when target samples come in one-by-one but it is still important to update the classifier even in the beginning when $\nq$ is very small?

We propose an label shift correcting estimator for which we can both provide generalization guarantees for an estimator which has access to the entire labeled source data and full or streaming access to unlabeled target data. 
% In this paper, we propose \ose, a principled method to exploit importance
% weights estimated on the source training set when we only have access
% to the covariates $x$ in the target set. 
% In short, our method, called \ose, e
Similar to~\citep{lipton2018detecting}, we first use a black-box classifier, which can be biased, uncalibrated and inaccurate, to efficiently estimate importance weights for the source samples. 
%we develop a statistically-efficient estimator for importance weighting. 
For classification tasks with $k$ classes, $\np$ labeled samples from the source and $\nq$ unlabeled samples from the target, we are able to estimate the importance weights with the square error upper bounded by $\wt{\mathcal{O}}\left(\sqrt{{\log(k)}/{\np}}+\sqrt{{1}/{\nq}}\right)$\footnote{$\wt{\mathcal{O}}$ is $O$ without $\log$ term on probabilities. With a slight abuse of notation, we denote $\wt{\mathcal{O}}\left(\cdot\right)+\wt{\mathcal{O}}\left(\cdot\right)$ as $\wt{\mathcal{O}}\left(\cdot+\cdot\right)$, as well as ${\mathcal{O}}\left(\cdot\right)+{\mathcal{O}}\left(\cdot\right)$ as ${\mathcal{O}}\left(\cdot+\cdot\right)$ }. This is an improvement over its predecessor method \citep{lipton2018detecting} which suffers from $k$ instead of $\log(k)$. Moreover, it removes the limiting warm-up sample complexity, the number of samples required for method to become applicable, in \citep{lipton2018detecting}.
%which is more robust to the growth in label size $k$. Consider the set of $r$ diseases, while each person can have any combination of these diseases, therefore, the number of labels $k=\mathcal{O}(r^r)$. We show that error in our estimator grows logarithmicly with $k$, i.e. $\log(k)$, therefore robust to even large class problems. 
Training on the source set with samples weighted by these estimated importance weights yields our
\ose estimator. We show that \ose generalizes well both in the streaming and batch setting. We derive a dimension-independent generalization bound for the \ose estimator and show that its excess risk is bounded by $\Rade_n+\wt{\mathcal{O}}\left(\sqrt{{\log(k)}/{\np}}+\sqrt{{1}/{\nq}}\right)$ where $\Rade_n$ is the complexity of function class used for the training. To the best of our knowledge, this the first generalization bound for label shift problems where no knowledge about the labels in the target domain is assumed. Furthermore, for the low sample regime, when $\nq$ or $\np$ are small, we deploy these bounds and develop a regularization method for the importance weight estimation and further improve our generalization bound. \fycomment{needs to be adjusted when we have a clear agenda for the $\lambda$} We empirically study the significance of \ose and show its performance under a variety of different shifts. 

==> Old_4-OSE.tex <==
\section{Regularized learning of label shifts (\ose)}
% We denote $\X$ as the space of input and $\Y$ as categorical space of labels $\Y=\left[k\right]=\lbrace 1,\ldots,k\rbrace$ as a set of classes/categories.  We express the joint distribution input-label $(x,y)\in \X\times\Y$ in source domain $\S$ as $\disP$ and in target domain $\T$ as $\disQ$. 
Let us denote the marginal probability mass functions of $Y$ for
$\disP, \disQ$ shorthand as $p, q: [k] \to [0,1]$ with $p(i) = \disP(Y
= i)$, and $q(i) = \disQ(Y= i)$ for all $i \in [k]$, representable by vectors in $\Real_+^k$ which sum to one. In label shift, the importance weights are as follows; $\forall i\in[k]$
\begin{align*}
\frac{\disQ(X,Y=i)}{\disP(X,Y=i)}=\frac{\disQ(X|Y=i)q(i)}{\disQ(X|Y=i)p(i)}=\frac{q(i)}{p(i)}
\end{align*}


We define $\weight\in\Re^k$ as the importance weight between these two domain $\weight(i)=\frac{q(i)}{p(i)}$. We quantify the shift with exponent of the infinite and second order Renyi divergence as follows
\begin{align*}
    d_\infty(q||p):=\sup_i\frac{q(i)}{p(i)}\quad, \quad\textit{and}\quad
    d(q||p):=\E_{(Y)\sim\disQ}\left[\weight(Y)Y\right]=\sum_i^k q(i)\frac{q(i)}{p(i)}
\end{align*}


\paragraph{Oracle approach: Weighting the training samples:}
A natural approach to correct for label shift is analogous to
weighting the samples by probability ratio in the covariate
shift setting.

Given a hypothesis class $\HH$, a loss function $\loss:\Y\times\Y\rightarrow [0,1]$ our aim is to find the hypothesis $h\in\HH$ which minimizes
\begin{align*}
    \LossPop (h) =\E_{(X,Y)\sim\disQ}\left[\loss(Y,h(X))\right] = \E_{(X,Y)\sim\disP}\left[\weight(Y) \loss(Y,h(X))\right]
\end{align*}
In the usual finite sample
setting however, $\LossPop$ unknown and we are given samples $\{(x_j, y_j)\}_{j=1}^n$ from $\disP$ instead. If we are given the vector of importance weights $\weight$ we could then minimize the empirical
loss defined as
\begin{align*}
    \LossPop_n (h)=\frac{1}{n}\sum_{j=1}^n \weight(y_j)\loss(y_j,h(x_j))
\end{align*}
where $n$ is the number of available observations used to learn the
classifier $h$.  In reality however, $\weight$ is unknown as well,
so that we are effectively finding the minimizer of
\begin{align}
  \label{eq:estimweightloss}
    \LossPop_n(h;\wh\weight)=\frac{1}{n}\sum_{j=1}^n\wh\weight(y_j)\loss(y_j,h(x_j))
\end{align}
where $\wh\weight$ are estimates of $\weight$.

We propose to use two-step procedure, given a set $\datap$ of $\np$ samples from
the source distribution $\disP$, we first divide the data set into two
sets where we use $(1-\beta)\np$ samples in set $\datapweight$ to
compute the estimate $\wh \weight$ and then the remaining $n= \beta
\np$ in the set $\datapclass$ to find the hypothesis which minimizes
the loss~\eqref{eq:estimweightloss}, i.e. $ \estweight = \argmin_{h\in \HH} \LossPop_n(h;\wh\weight)$.

In the following we describe how to estimate the
weights $\wh \weight$ and provide guarantees for the resulting
estimator $\estweight$.

\paragraph{Estimating weights while correcting for measurement error}

The following simple correlation between the label distributions $p,q$ was noted in~\citep{lipton2018detecting}: for a fixed hypothesis, if $\forall y\in \Y$, $q(y)\geq 0$, then $p(y)\geq 0$ $(\ast)$

it holds that for all $i,j\in\Y$, we have
\begin{align*}
    q_{h}(Y=i)&=\sum_j \disQ(h(X)=i|Y=j)q(j)=\sum_j \disP(h(X)=i|Y=j)q(j)\\
    &=\sum_j \disP(h(X)=i,Y=j)\frac{q(j)}{p(j)}=\sum_j \disP(h(X)=i,Y=j)\weight_j
\end{align*}
which can equivalently be written in matrix vector form (by slight abuse of notation) as
\begin{align}\label{eq:linear-model}
    q_{h}= \confmat_h \weight
\end{align}
where $C_h$ is the confusion matrix, that is $[C_h]_{i,j} = \disP(h(X)
= i, Y = j)$ and $q_h$ is the vector
which represents the probability mass function. The  is a reasonable setting since without any further prior knowledge, there is no way to properly reason about a class that does not exist in the source domain but appears in the target. The assumption $(\ast)$ considers a reasonable setting where without any further prior knowledge, there is no way to properly reason about a class in target domain that is not represented in the source domain. In general, both
$q_h$ and $\confmat_h$ can only be estimated by the corresponding
finite sample averages $\wh q_h, \wh\confmat_h$.

% In the paper~\citep{lipton2018detecting}, the authors simply use
% plug-in estimators and minimize $\|\wh \confmat_h \weight - \wh q_h\|_2$
% directly.  Although it is an optimal approach to solve a Gaussian noise model 
% when $\confmat_h$ is known to be precise,
% there is no theoretical justification to plug in a noisy
% $\wh \confmat_h$. Furthermore, when there are very few samples, the
% weight estimation will have high variance in which case it might
% be better to avoid importance weighting altogether. 

In the paper~\citep{lipton2018detecting}, the authors simply compute the inverse of $\confmat_h$ in order to estimate the importance weight, i.e. $\wh\confmat_h^{-1}\wh q_h$. This estimator could be considered as  statistically efficient estimator if the $ \confmat_h$ was known, i.e. $\confmat_h^{-1}\wh q_h$. While $\confmat_h$ is not known, this estimator can be arbitrary bad since the $\wh\confmat_h$ can be close to degenerate matrices. In order to relax this shortcoming, an additional problem dependent sample complexity is required to ensure that the estimator is away from degenerating. This sample complexity depends on the smallest singular value of $\confmat_h$ which is not known in advance, i.e. we can not specify when the estimator is valid. Despite requiring this knowledge, the resulting  error of this estimator is linear in $k$ which is sub-optimal and not suitable for when k is large. On the other hand, when there are very few samples, the weight estimation will have high variance in which case it might be better to avoid importance weighting altogether. 

Instead, we propose to use the following two-step procedure to compute
importance weights: Given a ``decent'' $(\ast\ast)$ black box estimator $\bbe$, we
\begin{enumerate}
\item calculate the measurement error adjusted $\thetaint$ as described in Section~\ref{sec:correctest} for $\bbe$,
compute the regularized weight $\wh \weight = \allones + \lambda \thetaint$ where $\lambda$ depends on the sample size $(1-\beta)\np$ and
  \item compute the minimizer $\estweight$ of the loss $\Loss_n(h; \wh\weight)$ in the hypothesis class $\HH$ with respect to $h$ 
\end{enumerate}
$(\ast\ast)$ Consider a $h_0$ almost always output a fix class, i.e. it does not capture any characteristics of the the data therefore no hope to gain any statistical information. As a consequence, a ``decent'' classifier $h_0$ is the one which does not result in any singularity in the spectrum of confusion matrix, i.e. $\confmat_{\bbe}$ is a full rank matrix.

In order to estimate the weights using the relationship in
equation~\eqref{eq:linear-model}, it is necessary to use some
prediction model, which we call $\bbe$, to begin with.  The choice of
the model determines the conditioning of solving both the oracle
population but also the finite sample version of
~\eqref{eq:linear-model}.  In the paper~\citep{lipton2018detecting},
it was assumed that $\bbe$ was a fixed a priori given black box
estimator which we have at our disposal and we will do the same.
Obviously in practice the black box estimator is not fixed and the
conditioning of $\confmat_{\bbe}$ determines estimation accuracy and
the computational complexity. We will further discuss the choice of an
appropriate initial black box estimation model $\bbe$ for implementation purposes in the experimental section.


\subsection{Estimator correcting for measurement errors}
\label{sec:correctest}
Both the design matrix and label distribution $\confmat_{\bbe},
q_{\bbe}$ on the target for black box hypthesis $\bbe$ are unknown and
we are only given finite sample estimates $\wh \confmat_{\bbe}, \wh
q_{\bbe}$.
% under the Gaussian assumption it is standard to use the
% total least squares approach which requires a single value
% decomposition. 
% \fycomment{Provide some explanation why we are not
%   doing it here}
% We use a different approach which targets the same type of measurement
% errors. 
Note that in what follows all empirical and population
confusion matrices as well as label distributions are defined with
respect to the hypothesis $h = \bbe$.  For notational simplicity, we
thus drop the subscript $\bbe$ in  what follows.

In the unweighted case $\weight = \allones$, and thus the amount of weight shift
is captured in $\theta = \weight - \allones$. The reparameterized linear model~\eqref{eq:linear-model} with respect to $\theta$ then reads
\begin{equation*}
   b:= q - \confmat \allones = \confmat \theta
\end{equation*}
with corresponding finite sample quantity $\wh b = \wh q - \wh \confmat \allones$. 
When $\wh \confmat$ is near singular, the estimation of $\theta$ becomes unstable.
Furthermore, small values in the true weight $\weight$ result in large variances.
We address this problem by adding a regularizing $\ell_2$ penalty term to the usual loss
and thus push the amount of shift towards $0$, a method that has been proposed in \citep{pires2012statistical}.
In particular, we compute
\begin{equation}
  \label{eq:weightint}
  \thetaint = \argmin_{\thetaint_\rho: \rho \in \{2^{i+1}\Delta_C \Delta_b, i\in \NN\}} \|\wh \confmat \thetaint_{\rho}- \wh b\|_2 + 3 \Delta_C \|\thetaint_{\rho}\|_2
\end{equation}
%% We consider the weight estimate 
%% \begin{equation}
%%   \label{eq:weightint}
%%   \weightint = \argmin_{\weightint_\rho \in \{2^{i+1}\Delta_C \Delta_q, i\in \NN\}} \|\wh \confmat \weightint_{\rho}- \wh q\|_2 + 3 \Delta_C \|\weightint_{\rho}-1\|_2
%% \end{equation}
where $\thetaint_\rho$ is defined by 
\begin{equation}
  \thetaint_\rho = \argmin_{\theta'} \| \wh\confmat \theta' - \wh b\|^2_2  + \rho \| \theta'\|_2.
\end{equation}

Here, $\Delta_C, \Delta_b$ are parameters which will then be chosen to
be high probability upper bounds for $\|\wh \confmat - \confmat\|_2$
and $\|\wh b- b\|_2$ respectively.  Let $\sigma_{\min}$ be the minimum
singular value of the true confusion matrix $\confmat$.  For the
estimate $\thetaint$ we have the following upper bound

\begin{lemma}
\label{lem:weightest}
For $\thetaint$ as defined in equation~\eqref{eq:weightint}, we have with probability at least $1-\delta$ that
\begin{align*}
  \|\thetaint-\theta\|_2\leq
  \bigo \left( \frac{1}{\sigma_{min}}\big( (\|\theta\|_2)\sqrt{\frac{\log (k/\delta)}{(1-\beta)\np}}+\sqrt{\frac{\log (1/\delta)}{(1-\beta)\np}} + \sqrt{\frac{\log(1/\delta)}{m}}\big)\right)
  %% \frac{1}{\sigma_{min}}\left(\frac{2\|\weight\|_2}{(1-\beta)\np}+\|\weight\|_2\sqrt{\frac{18\log\left(4k/\delta\right)}{(1-\beta)\np}}+\sqrt{\frac{36\log\left(2/\delta\right)}{m}}\right)
\end{align*}
where $\delta < 0.5$.
\end{lemma}
% \fycomment{I summarized the $\log k$ and $\|\theta\|_2$ term ...}

%\fycomment{still need definition of $\bigo$ etc.}
Here, we hide universal constants in the $\bigo$ notation. Furthermore, 
we use $\bigo \left(\cdot+\cdot\right)$ for short to denote $\bigo \left(\cdot\right)+ \bigo \left(\cdot\right)$.

A couple of remarks are in order at this point.
First of all, notice that the upper bound in Lemma~\ref{lem:weightest} includes $\sigma_{\min}(\confmat)$ as a parameter, apart from the norm of the true weight shift $\theta$. Recall that these quantities are all heavily dependent on the
black box estimator $\bbe$ that we are given a priori. In particular, if $\bbe$ is an ideal estimator, and the source
set is balanced, $\confmat$ is the unit matrix with $\sigma_{\min}=1/k$. In contrast, when the model $\bbe$ is uncertain, the singular value $\sigma_{\min}$ is close to zero. 

The choice of the $\theta$ estimator: Generally, for least square problems, where the goal is to minimize the square of loss, under the Gaussian assumption, it is standard to use regularized total least squares approaches which requires a single value decomposition. In this work, we deploy an alternative estimator, Eq.~\ref{eq:weightint}, a hyperparameter free estimator where neither loss nor regularization is squared. This choice of estimator is motivated in label shift problems, where the $\theta$ vector can be big and squared regularization might cause a big and undesired amount of regularization away from the true parameter \citep{pires2012statistical}.


% under the Gaussian assumption it is standard to use the
% total least squares approach which requires a single value
% decomposition. 
% \fycomment{Provide some explanation why we are not
%   doing it here}
% We use a different approach which targets the same type of measurement
% errors. 

\fycomment{Discuss the choice of $\rho$ in real implementations...}
%% \begin{theorem}[Generalization bound for $\est_{\weightint}$]
%% \label{thm:genbound}
%% Given a finite hypothesis class $\HH$ with cardinally of $|\HH|$, $n$ sample from the source data set, $m$ sample input from target set results in the following generalization bound.
%% \begin{align}\label{eq:Lhatwhat}
%%   |L(\est_{\weightint})-L(h^*)|
%%   &\leq
%%   2 \Rade_n(\G) + \dismaxpq \sqrt{\frac{\log 2/\delta}{n}} \\
%%   &+ O \left( \frac{1}{\sigma_{min}}\big( \|\weight\|_2 \sqrt{\frac{\log (k/\delta)}{(1-\beta)\np}} + \sqrt{\frac{\log(1/\delta)}{m}}\big)\right)\nonumber

%% \end{align}
%% with probability at least $1-\delta$ where $\delta\leq 0.5$.
%% \end{theorem}

\subsection{Regularized estimator and generalization bound}
When the number of samples in the target set or the shift is very low,
for example in the scenario where the estimated weights might be too
uncertain to be applied.  We therefore propose a regularized estimator
to correct for label shift in the anti-causal learning which is defined as follows
\begin{equation}
\label{eq:finalweight}
%  \wh \weight = (1 - \lambda)\textbf{1} + \lambda \weightint.
    \wh \weight = \textbf{1} + \lambda \thetaint.
\end{equation}
Intuitively, by rewriting $\wh\weight =(1 - \lambda)\textbf{1} + \lambda (\allones + \thetaint)$, 
we see that $\lambda$ closer to $1$ the more reason to belief that
$\allones + \thetaint$ is in fact the true weight. 
Notice that $\wh \weight$ implicitly depends on $\lambda, \beta$.  Given the estimation we can bound the generalization error.
% If
% we now use $\wh \weight$ to compute $\estweight$ with $n = \beta \np$,
% we can bound the generalization error using two key quantities
% \begin{equation}
%   \dispq := \E_{\disP} \weight^2(Y) = \sum_{i=1}^k q(i)\frac{q(i)}{p(i)} \qquad \text{and } \qquad \dismaxpq = \sup_i \frac{q(i)}{p(i)}.
% \end{equation}
 In the following we state a another bound on the general hypothesis classes. Let's define a set $\G(\loss, \HH) = \{g_h(x,y) = w(y) \loss(h(x),y): h\in\HH\}$, under $n$ data points and loss function $\loss$. Consider the typical Rademacher complexity measure for the size of a hypothesis class $\HH$ as  $\Rade_n(\G) := \E_{X(i),Y(i)\sim\disP:i\in[n]}\left[\E_{\sigma_i:i\in[n]}\frac{1}{n}\left[\sup_{h\in\HH}
\sum_{i=1}^n \sigma_i \weight(y_i) \loss(x_i, h(y_i))\right]\right]$.


\begin{theorem}[Generalization bound for $\estweight$]
\label{thm:genbound}
Given $n$
sample from the source data set and $m$ sample input from target set, a hypothesis class $\HH$ with Rademacher complexity $\Rade_n(\G)$ under $\loss$
results in the following generalization bound.
\begin{align}\label{eq:Lhatwhat}
  |\Loss(\estweight)-\Loss(h^*)|&\leq
  2 \Rade_n(\G) + \dismaxpq \sqrt{\frac{\log (2/\delta)}{n}}+ \left(1-\lambda\right)\|\theta\|_2\\
  &+\frac{\lambda}{\sigma_{\min}} \bigo \Bigg(\|\theta\|_2 \sqrt{\frac{\log\left(6k/\delta\right)}{(1-\beta)\np}}
  +\sqrt{\frac{\log\left(3/\delta\right)}{(1-\beta)\np}}
  +\sqrt{\frac{\log\left(3/\delta\right)}{\nq}}\Bigg) \nonumber
\end{align}
with probability at least $1-\delta$ where $\delta\leq 0.5$.
\end{theorem}

The proof can be found in Section~\ref{proof:genbound}.

% \fycomment{re Kamyar: yeah we can get a better dependence on $p,q$ (that is $\dismaxpq$ for finite
%   hypothesis class with union bound and Bernstein $\dispq$ but 1. it's not
%   the main point so I'm glossing over it here, 2. we usually don't have finite classes in application so why show it for that particular case}
%  \Kamyar{Please bring back the d and the discussion I had on it. The same union bound used for finite function class aslo holds for Rademacher. Also, other stuff in the draft I wrote, please bring those also back. No need to have all of them in the main text, but  have them all in the apx.}
%  \fycomment{I'm open to discussion, but please be more specific what exactly you are missing, see email. Your original writing is untouched in the tex files (I only commented them out) you may add back whatever you like as long as notation  flow stay consistent and no unnecessary lemmas/steps are added.}

How large $\Rade_n(\G)$ is determined by the function class and
depends on the structure of $\HH$ and the loss $\loss$. 
For example
for the $0/1$ loss, the VC dimension of $\HH$  can be deployed to upper bound the Rademacher complexity.

We further extend the analysis in Theorem.~\ref{thm:genbound} and provide a tighter bound of $\wt{\mathcal{O}}(\frac{\dismaxpq}{n}+\sqrt{\frac{\dispq}{n}})$ for finite hypothesis class (look at ~\ref{proof:genbound-finite}). %which is also extendable to general hypothesis classes.


% \fycomment{Discuss how $\weight$ comes in, something like Kamyar's text below}
% To parse this bound, as we can see, it no more depends on $\|\omega\|_2$ rather to $\|\textbf{1}-\weight\|_2$ which goes to zero in low shift setting, also the regularization in Eq.~\ref{eq:theta-rho} and \ref{eq:thetahat-optimal} tend to make the importance weights close to no shift setting. Another super interesting characteristics of this bound is in its dependency on cardinality of label space, $k$. This dependency appears as $\log(k)$ which allows for larger label sizes. It means for multi-label classification, e.g. each person can have multiple diseases at once, while we should be careful about possible growth of $\|\theta\|_2$. 

% \fycomment{Discuss role of $\beta,\lambda$, something like Kamyar's text below}
% Now there are two main question left. First is the choice of $\beta$ which needs to be chosen a priori from the set $\B$ (before applying the final classifier on the target domain). Second one is the case when the number samples in the source and target are fairly small, and also the shift induced by $\theta$ is big or small.

In order to use Theorem~\ref{thm:genbound} in practice, with ideal
$\lambda, \beta$, we need to assume some a priori knowledge of an
upper bound $\thetamax$ of the possible shifts we might encounter, i.e.
\begin{equation}
  \label{eq:maxweight}
  \|\theta\|_2 \leq \thetamax.
\end{equation}
and we consider the following cruder bound instead for 
practical implementation
\begin{align}\label{eq:Lhatwhatmax}
  |\Loss(\estweight)-\Loss(h^*)|&\leq
  2 \Rade_n(\G) + \dismaxpq \sqrt{\frac{\log (2/\delta)}{\beta\np}}+ \left(1-\lambda\right)\thetamax\nonumber\\
  %% \frac{2 \dismaxpq \left( \log(|\HH|)+\log(\frac{3}{\delta})\right)}{3\beta \np}+\sqrt{\frac{8\left(\dispq\right)\left(\log(|\HH|)+\log(\frac{3}{\delta})\right)}{\beta \np}}\nonumber\\
    %% &+\frac{\lambda}{\sigma_{min}}\Bigg(\frac{2\|\theta\|_2\log\left(3k/\delta\right)}{(1-\beta)\np} \\
  %% &\quad\quad\quad~~+\|\theta\|_2\sqrt{\frac{18\log\left(6k/\delta\right)}{(1-\beta)\np}}+\sqrt{\frac{36\log\left(3/\delta\right)}{(1-\beta)\np}}+\sqrt{\frac{36\log\left(3/\delta\right)}{m}}\Bigg)
  &+\frac{\lambda}{\sigma_{\min}} \bigo \Bigg(\thetamax \sqrt{\frac{\log\left(k/\delta\right)}{(1-\beta)\np}}
  +\sqrt{\frac{\log\left(3/\delta\right)}{(1-\beta)\np}}
  +\sqrt{\frac{\log\left(3/\delta\right)}{\nq}}\Bigg)
\end{align}
\begin{wrapfigure}{t}{.3\textwidth}
\caption{Given a $\sigma_{\min}$ and $\theta_{\max}$, $\lambda$ switches from $0$ to $1$ at a particular $\nq$. $\np$ is kept fixed.}
  \centering
  \footnotesize
  \includegraphics[width=0.9\linewidth]{figs/threshold.eps}
%   \label{table:settings}
\vspace*{-1.5cm}
\end{wrapfigure}

The bound~\eqref{eq:Lhatwhatmax} gives us guidance as to how to choose $\lambda$ as a function of the number of samples in practice. Notice that both $\thetamax$ and $\sigma_{min}$ are unknown. 
When $\nq \geq \frac{1}{\thetamax^2(\sigma_{\min} - \frac{1}{\sqrt{n}})^2}$ the best choice is $\lambda = 1$. However since $\thetamax$ is just an upper bound on the true amount of shift $\|\theta\|_2$, when
\begin{equation*}
\frac{1}{\thetamax^2(\sigma_{\min} - \frac{1}{\sqrt{n}})^2} \leq \nq \leq \frac{1}{\|\theta\|_2(\sigma_{\min} - \frac{1}{\sqrt{n}})^2}
\end{equation*}
$\lambda$ should in fact ideally be $0$. 
Thus for $\nq$ that are barely below the threshold, it could be sensible 
to use an intermediate value. 


% \fycomment{how about the following paragraph instead? I would not put the table, but it's good to put the discussion in the tex.}\Kamyar{can you tell me how to derive it?}\fycomment{never mind, doesn't make much sense right now...}
% As mentioned above, $\lambda$ intuitively corresponds to how much we believe the weight estimate $\allones + \thetaint$ to be close to the true weights and how important the weight correction is, i.e. how large the amount of shift is.
% If $\lambda$ is now chosen to be $\max \{ \min \{ 1 - \bigo (\frac{1}{\sqrt{\np}} +\frac{1}{\sqrt{\nq} \thetamax}), 1\}, 0\}$ as a function of the amount of shift and the set cardinalities, the generalization error then scales with
% \begin{equation*}
% 2 \Rade_n(\G) + \sqrt{\frac{\dismaxpq^2}{\beta \np}} +  \bigo \big(\sqrt{\frac{\thetamax^2}{(1-\beta) \np}} +  \sqrt{\frac{1}{\nq}} \big)
% \end{equation*}
% where we omitted log terms, $\sigma_{\min}$. 
% This choice of $\lambda$ aligns with the intuition that the larger the source and target set, the, the more weight we can put on the estimated importance weights, i.e. $\lambda$.
% We can also see the trade-off between the amount of shift $\thetamax$ and the sample size of the target set $\nq$: When either of them is large, the importance weight correction is either more reliable or more important.


% \paragraph{On the choice of $\lambda$}
% The proper choice of $\lambda$ depends on the maximum amount of shift $\thetamax$ that is known or believed to be true, as well as the sample sizes of the source and target set $\np$, and $\nq$. In a desired setting, when $\thetamax$ is fairly small while both $\np$, and $m$ are large,  setting $\lambda =1$. Intuitively, when shift is not significant while we have few samples from the target domain, it is better to deploy a trained classifier on the source, with no importance weight involved, i.e. $\lambda\rightarrow 0$. On the other hand, when the shift is big, but we have many samples from target, we have a good estimation of the importance weight vector and would like to use it as it is, i.e. $\lambda\rightarrow 1$. An interesting situation is when the shift is significantly large. In this scenario, even if a couple of samples from target domain are accessible, they are informative enough to make us to use the estimated importance weight vector as it is, i.e. $\lambda\rightarrow 1$

% \newcolumntype{?}{!{\vrule width 2pt}}
% % \begin{table*}[h]
% \begin{wrapfigure}{t}{.35\textwidth}
% % \caption{On choices of $\lambda$}
% % \begin{minipage}{1.\textwidth}
%   \centering
%   \footnotesize
%   \begin{tabular}{c?c?c}
%     % \multicolumn{1}{c}{Covariate Shift }&\multicolumn{1}{c}{Label Shift} \\
%     % \toprule
%  $\thetamax \downarrow$& $m\downarrow$&$\Longrightarrow \lambda\rightarrow 0$\\
%     \specialrule{.1em}{.05em}{.05em} 
% $\thetamax \uparrow$&  $m\uparrow $&$\Longrightarrow \lambda\rightarrow 1$\\
% % \midrule
% \specialrule{.1em}{.05em}{.05em} 
% $\thetamax \uparrow\uparrow$& $m\downarrow $&$\Longrightarrow \lambda\rightarrow 1$\\
%     % \bottomrule
%   \end{tabular}
% %   \vspace*{-.5cm}
% %   \label{table:settings}
% % \end{minipage}
% % \end{table*}
% \end{wrapfigure}

% These intuitive paradigms also matches the claims captured in Theorem.~\ref{thm:genbound} and Eq.~\ref{eq:Lhatwhatmax}. For the case of significantly large shift, if the number of samples from the source domain, $\np$ 
% , is also small, then the task is almost impossible to approach. This is also captured by the bound since the RHS of Eq.~\ref{eq:Lhatwhatmax} is larger than one, therefore, vacuous. There are scenarios in between where we prefer $0\leq\lambda\leq 1$. 


% is small, the right hand side 
% Intuitively, when the number of samples in the target domain, $m$, is low, the last term in the Eq.~\ref{eq:Lhatwhatmax} grows. Consider the case where $\thetamax$ is small, then we intuitively prefer to do not use our estimated $\wh \weight$ and just use the a good classifier trained directly on the source data to use against target data. On other hand, consider the case where $\thetamax$ is large. In this setting, since the shift is big, even a signal sample from the target domain is highly helpful and informative to enhance the classifier by far. In this setting we like to fully use the estimated $\wh\weight$ to train the suitable classifier against target set. There are setting in between that we might like to regularize the estimated importance weights $\wh \weight$ a bit toward shift setting. We introduce $\lambda$- shifted importance weight as $\wh\weight=\textbf{1}+\lambda \wh \theta$, with $0\leq\lambda\leq 1$. For this case, $\lambda=0$ means regularize all the way to no shift setting, while $\lambda=1$ means to keep the weights as they are and no further regularization. We consider the setting with a set of possible $\lambda$'s from a finite set of $\Lambda$ which we can chose $\lambda$ a priori. Therefore, putting these two components of the generalization together we get;




% $\lambda^*\approx\max\lbrace 0,\min\lbrace \thetamax-\mathcal{O}(\thetamax/\sqrt{n})-\mathcal{O}(1/\sqrt{n})-\mathcal{O}(1/\sqrt{m}),1\rbrace\rbrace$

% A simple manipulation shows that the optimal $\lambda$ is either zero or one. Since the bound is constructed for worst case scenario, in order to choose a useful $\lambda$ for practice, we follow the Bayesian interpretation of this bound. In practice we do not have $\theta_{\max}$ but just a belief of it and also the concentration bounds also follow  Bayesian posteriors which results in $\lambda$ between zero and one.
% Then the useful lambda has an interesting behaviour with respect to the detail parameters, i.e. $\lambda^*\approx\max\lbrace 0,\min\lbrace \thetamax-\mathcal{O}(\thetamax/\sqrt{n})-\mathcal{O}(1/\sqrt{n})-\mathcal{O}(1/\sqrt{m}),1\rbrace\rbrace$.%\footnote{Since we have a linear program on the solution is either zero or one but in practice we do not have $\theta_{\max}$ but just a belief of it and also the concentration bounds can also become Bayesian which results in $\lambda$ between zero and one.}



\subsection{Regularized estimator for the streaming setting}

Consider a situation where we send a group of volunteers to a new
country with new disease distribution of dangerous disease. In this case we do not have time to wait to collect enough
samples in order to train a classifier. We are interested in updating
our model more often, even maybe after visiting any new patient. 

% Note that the regularization enables us to update our classifier $h$
% in settings where we only have few samples in the target set, e.g. when we
% have only observed symptoms from very few patients in a different
% country.

%% \ose estimates the importance weights $\weight$ in a principled way by solving multiple small convex problems Then uses the estimated weight to train a classifier. 
We thus propose to use the following algorithm in the streaming
setting when at time $t$ we have acquired $t$ unlabeled samples from
the target set. The key is that we can choose both $\beta^\star, \lambda^\star$ at any
time step depending on $t$, described in the algorithm below.

\input{algorithm}
%\fycomment{the $\lambda^\star$ in the algorithm is probably not the actual minimization (since that would be $0,1$) but the heuristic you described above...}

Note: Obviously it is very costly to compute both $\lambda^\star, \beta^\star$ and recompute the classifier after each new sample is obtained. We want to emphasize that the steps in the loop can be skipped as desired and as the budget allows, e.g. recompute after a batch of data arrives. The accuracy guarantees given in  Corollary~\ref{cor:streaming} still hold.


The generalization bound for $\estweight$ in this setting directly follows from
Theorem~\ref{thm:genbound} and the union bound.
\begin{corollary}[Generalization Bound for the streaming setting]
\label{cor:streaming}
For the estimator $\estweight^t$ in Algorithm~\ref{alg:ose} after running $\ose$ for $t$ time steps 
we obtain the following upper bound on the generalization error
%   Given a finite hypothesis class $\HH$ with cardinally of $|\HH|$,
%   $\np$ samples from the source data set, splitting set $\B$,
%   regularization set $\Lambda$, after $t$ time steps of running \ose, and $t$
%   observations from the target domain, we have
\begin{align}\label{eq:finalbound}
  |\Loss(\estweight^t)-\Loss(h^*)|&\leq
  2 \Rade_n(\G) + \dismaxpq \sqrt{\frac{\log (2t/\delta)}{n}}+ \left(1-\lambda\right)\|\theta\|_2\\
  &+\frac{\lambda}{\sigma_{\min}} O\Bigg((\|\theta\|_2)\sqrt{\frac{\log\left(kt/\delta\right)}{(1-\beta)\np}}+\sqrt{\frac{\log\left(t/\delta\right)}{(1-\beta)\np}}
  +\sqrt{\frac{\log\left(t/\delta\right)}{t}}\Bigg) \nonumber
\end{align}
with probability at least $1-\delta$ when $\delta<0.5$.
\end{corollary}



==> algorithm.tex <==
\algnewcommand{\IIf}[1]{\State\algorithmicif\ #1\ \algorithmicthen}
\algnewcommand{\EndIIf}{\unskip\ \algorithmicend\ \algorithmicif}

\begin{algorithm}[ht]
\caption{\ose in the streaming setting}
\begin{algorithmic}[1]
\State Input: source set $\datap$, $\dataq:\emptyset$, $\thetamax$, black box estimator $\bbe$, model class $\HH$
\For{t = 1 to $T$}
    \State $\dataq\leftarrow \dataq\cup x_t$, then determine optimal split ratio $\beta^*$ by minimizing the RHS of Eq.~\ref{eq:Lhatwhat} 
    \State Randomly partition source set $\datap$ into $\datapclass, \datapweight$ such that $|\datapclass| = \beta^*\np =: n$ 
    \State Compute $\thetaint$ using Eq.~\eqref{eq:weightint}
    \State Determine $\lambda^*$ by minimizing the RHS of Eq.~\ref{eq:Lhatwhatmax} and compute $\wh \weight:= 1 + \lambda^\star \thetaint$
    \State Minimize the importance weighted empirical loss  to obtain the weighted estimator
    \begin{align*}  
\estweight^t =\arg\min_{h\in\HH}\Loss_n(h;\wh\weight),\qquad \textit{where} \qquad  \Loss_n(h;\wh\weight)=\frac{1}{n}\sum_{(x,y)\in \datapclass}\wh\weight(y)\loss(y,h(x))    
    \end{align*}
% 	\IIf {count mod $T^{sample}~ = ~0$}
%     	 sample $W\sim\mathcal{N}\left(W^{target},Cov\right)$
%     \EndIIf
    \State Deploy $\estweight^t$ if the risk is acceptable
\EndFor
\end{algorithmic}
\label{alg:ose}
\end{algorithm}

